Optimal personalised treatment computation through in silico clinical trials on patient digital twins

In Silico Clinical Trials (ISTC), i.e., clinical experimental campaigns carried out by means of computer simulations, hold the promise to decrease time and cost for the safety and efficacy assessment of pharmacological treatments, reduce the need for animal and human testing, and enable precision medicine. In this paper we present methods and an algorithm that, by means of extensive computer simulation--based experimental campaigns (ISTC) guided by intelligent search, optimise a pharmacological treatment for an individual patient (precision medicine). e show the effectiveness of our approach on a case study involving a real pharmacological treatment, namely the downregulation phase of a complex clinical protocol for assisted reproduction in humans.

==> 00.database/content.tex <==
% !TEX root =  ../root.tex

\DataPut{exps/treatment day min start}{\Pretty{21}}
\DataPut{exps/treatment day max start}{\Pretty{25}}

\DataPut{exps/results/clinicalrecords/datasets}{Pfizer Inc.\ and Hannover Medical School (Germany)}
\DataPut{exps/results/clinicalrecords/all}{\Pretty{21}}
\DataPut{exps/results/clinicalrecords/measurements/all}{\Pretty{800}}

\DataPut{exps/results/population}{\Pretty{e7}}


\DataPut{exps/results/mape}{\Pretty{35}\%}
\DataPut{exps/results/computation/dt/size/avg}{\Pretty{843424}}
\DataPut{exps/results/computation/dt/clusters/num/avg}{\Pretty{11}}
\DataPut{exps/results/computation/time/avg/days}{\Pretty{15} days}
\DataPut{exps/results/computation/simtime/avg/perc}{\Pretty{81.20}\%}
\DataPut{exps/results/computation/correlation/dt nodes}{\Pretty{-60}\%}

\DataPut{exps/results/average dose}{\Pretty{40.82}\%}
\DataPut{exps/results/average dose saving}{\Pretty{59.18}\%}
\DataPut{exps/results/stddev}{\Pretty{13}\%}


%% Size of sub-figures
\DataPut{paper/figures/subfigures/cols/2/width}{0.48\linewidth}
\DataPut{paper/figures/subfigures/cols/3/width}{0.31\linewidth}

==> 01.introduction/content.tex <==
%!TEX root = ../root.tex

\Input{framework.tex}

\subsection{Motivations}
\label{sec:motivations}
\Input{motivations.tex}

\subsection{Contributions}
\label{sec:contributions}
\Input{contributions.tex}




==> 01.introduction/contributions.tex <==
%!TEX root = ../root.tex

In this paper we present methods and an algorithm that, by means of extensive computer simulation--based experimental campaigns (\Aclp{ISCT}, \Acsp{ISCT}) 
\AcronymUsed{ISCT}%
guided by intelligent search, optimise a pharmacological treatment for an individual patient. 
We show the effectiveness of our approach on a case study involving a real pharmacological treatment, namely the \emph{downregulation} phase of a complex clinical protocol for assisted reproduction in humans. 

To do this, we exploit a state-of-the-art \Ac{VPH} model of the \Ac{HPG} axis (whose accuracy has been experimentally assessed in \cite{roeblitz-etal:2013:theorbio}) in order to conduct an \Ac{ISCT}.
%
Namely, starting from clinical data collected from a real patient, we first compute her \emph{\digitaltwin}, which defines a \emph{digital} representation of \emph{that} patient physiology.
%
%
Then, we compute \insilico, by means of intelligent search on such a \digitaltwin, the lightest (in terms of overall amount of administered drug) treatment still effective for that patient.

Our search algorithm extends standard artificial intelligence techniques (such as, \eg classical planning~\cite{weld:1999:planning}, CSP~\cite{rossi-etal:2006:constraint} and SAT~\cite{biere-etal:2009:sat}) in order to
% drive a simulator of the \Ac{VPH} model at hand to
\emph{intelligently} explore the space of possible time-series of drug administrations (treatments)
by driving a simulator of the \Ac{VPH} model at hand.
To improve the performance of our search algorithm, we also define suitable ordering heuristics (which keep our approach complete) and we evaluate their marginal performance gain.
%
Moreover, our implementation can be easily adapted to several \Ac{VPH} models and to a wide class of clinical treatments as it drives a Modelica black-box simulator.

In order to assess the technical viability of our approach,
we
exploit the above \Ac{HPG} axis \Ac{VPH} model to
conduct a multi-arm \Ac{ISCT} involving 
\DataGet{exps/results/clinicalrecords/all} 
patients (for which we have retrospective clinical measurements).
For each such patient, who defines a distinct arm of our \Ac{ISCT}, we compute the optimal (lightest) still-effective downregulation treatment.
Given that the required computation is extremely intensive, we conduct our \Ac{ISCT} on a large \Ac{HPC} infrastructure.

The possibility to \emph{optimise} \insilico a complex treatment for a given human patient \emph{before} its actual administration shows the potential of artificial intelligence search methods for model-based (\insilico) medicine. 


\subsubsection*{Paper outline} 
The paper is organised as follows.
\Cref{sec:preliminaries} describes some background knowledge, introduces the \Ac{HPG} axis model used in our case study and its phenotypes, defines the concept of clinical record and that of \digitaltwin of a human patient.
\Cref{sec:treatment} describes the treatment we used as our case study.
In \cref{sec:computing} we describe our algorithm to find optimal personalised treatments by means of intelligent search which drives a black-box simulator of a patient \digitaltwin. 
\Cref{sec:experiments} describes our experimental campaign on retrospective data and analyses the outcome of our multi-arm \Ac{ISCT}. 
Finally, \cref{sec:state-of-the-art} discusses related work and \cref{sec:conclusions} draws conclusions.


==> 01.introduction/framework.tex <==
%!TEX root = ../root.tex

\emph{Model-based} approaches to safety and efficacy assessment of
pharmacological treatments (\Aclp{ISCT}, \Acsp{ISCT}) 
\AcronymUsed{ISCT}%
hold the promise to \emph{decrease} time and cost for the needed experimentations, \emph{reduce} the need for animal and human testing, and enable \emph{precision} medicine, where \emph{personalised} treatments \emph{optimised} for each patient can be designed before being actually administered.
%
This is to be achieved by developing \emph{computational models} for human physiology, patho-physiology, and drugs \Ac{PK} and \Ac{PD}.
Such computational models also define the possible physiological differences between different individuals and/or different reactions to drug administration. In particular, \Ac{PK} and \Ac{PD} models describe drug concentrations and effects over time in the human body (see, \eg \cite{mould-etal:2012:pkpd}), \respectively.

Encapsulating knowledge of the human physiology into computational models is among the goals of \Ac{VPH} (see, \eg~\cite{clapworthy-etal:2007:vph}).
Indeed, research in \Ac{VPH} provides mechanistic quantitative models of the human
physiology at different levels of scale and for various medical areas
(\eg~cardiology, endocrinology, oncology and neurology, see~\cite{trayanova-etal:2018:curr-opin-biomed-eng,cox-etal:2009:circulatory, roeblitz-etal:2013:theorbio, ribba-etal:2012:tumor, jackson-etal:2015:neuro}).
For example, several models have been proposed for \emph{molecules} (\eg
\cite{roy-etal:2010:jpp}), cells (\eg
\cite{bachler-etal:2014:species,iarosz-etal:2015:jtb}) and single organs (\eg \cite{yalcinkaya:2013:eleco,cox-etal:2009:circulatory,muller:2014:ijnmbe}).
%
At upper levels in the hierarchy, we find models of human body \emph{compartments}. 
Good examples are models in \cite{kanderian-etal:2009:jdst,herrero-etal:2013:jdst,dallaman-etal:2014:jdst}, which define the glucose regulation mechanism in patients with Type 1 Diabetes Mellitus, and the \Ac{HPG} axis model presented in \cite{roeblitz-etal:2013:theorbio}, which is specifically focused on hormones related to the human menstrual cycle. 
%
Finally, at the top level we find models of the \emph{whole human} body, for example the Glucose-Insulin Model~\cite{schaller-etal:2013:glucose,schlender-etal:2016:clinpharm}, HumMod~\cite{hester-etal:2011:frontphysiol}, and Physiomodel~\cite{matejak-etal:2015:embc}.

Independently of the level of scale used, most \Ac{VPH} models are defined by means of complex, highly non-linear differential equations. By means of numerical integration, such models can be executed within \emph{simulators} in order to provide quantitative information about the time evolution of the modelled biological quantities (\eg blood hormone or glucose concentrations).

\Ac{VPH} models at different positions in the above hierarchy are typically defined at different levels of abstraction.
In order to find a trade-off between simulation accuracy and efficiency, \emph{multi-scale} models can be built by integrating, interconnecting, and co-simulating models of the different organs or body compartments of interest, exploiting the different available levels of abstraction as required by the focus and scope of the \insilico analysis to be performed.

Different languages are traditionally used to define \Ac{VPH} models. Among them are \Ac{SBML} \cite{hucka-etal:2003:bioinf} and \Ac{PHML} (see, \eg \cite{yoshiyuki-etal:2014:phml}). 
The Modelica language (\url{http://www.modelica.org}), one of the most widely adopted open-standard general-purpose modelling languages for networks of dynamical systems within many areas of engineering, has been proposed as a common modelling platform for the integration of \Ac{VPH}, \Ac{PKPD} models as well models for engineered systems such as biomedical devices (see, \eg \cite{fritzson-etal:2007:biochem,maggioli-etal:2019:bioinf}) in order to facilitate their co-simulation and analysis.





==> 01.introduction/motivations.tex <==
%!TEX root = ../root.tex

Current pharmacological treatments are often designed with the \emph{average} patient in mind. 
A key topic in \emph{precision medicine} is to develop pharmacological treatments \emph{optimised} for any given individual, namely \emph{personalised} treatments (see, \eg \cite{avicenna:2016:roadmap,pappalardo-etal:2018:insilico}). 
Several optimisation criteria can be defined. A typical criterion is the minimisation of the overall amount of drug used,
which often also reduces the probability of adverse side-effects and contributes to decrease the treatment cost.

With their amenability to define different individuals, \Ac{VPH} models of proved accuracy are a \emph{key enabler} for precision medicine. 


==> 02.state-of-the-art/content.tex <==
%!TEX root = ../root.tex
%
Individualised treatments have the potential value to reduce costs and improve
outcomes of standard clinical treatments.
In recent years data-driven techniques have been investigated thanks to the
availability of big data \cite{raghupathi-etal:2014:hiss}.
For example, the knowledge-base approach in \cite{fogliata-etal:2014:radonc} has been used to
optimise treatment plans for lung cancer.
Unfortunately, in presence of scarce clinical data for the patient at hand, the above approaches cannot
be applied. For example, in our case study hormones blood concentrations are not measured every day, since those measurements are costly and invasive.

Model-based approaches, exploiting \Ac{PK}, as \eg
\cite{willmann-etal:2003:biosilico}, are used instead to
build populations of virtual phenotypes. Such populations are used to optimise and individualise drug doses \cite{jeena-etal:2011:aac,dijkman-etal:2018:cpt}.
\Ac{PK}-based models, however, do not define how administered drugs can
affect a \Ac{VP} (namely, \Acl{PD}, \Acs{PD}), 
\AcronymUsed{PD}%
\ie possible side-effects due to drug administrations are not taken into account.

In our model-based setting, we have to face with complex \Ac{VPH}
models, \eg HumMod \cite{hester-etal:2011:frontphysiol},
Physiomodel \cite{matejak-etal:2015:embc}, and
GynCycle \cite{roeblitz-etal:2013:theorbio}
defined through highly non-linear differential equations modelling the underlying biological mechanisms (\eg inhibitory and stimulatory effects).
%
As outlined in \cref{sec:computing:model}, such \Ac{VPH} models are hybrid systems
that can be defined by systems of \Acp{ODE} (see, \eg \cite{lenovere:2015:nrg,bartocci-etal:2016:plos-comp-bio,wang-etal:2016:hldvt}) whose inputs are discrete event sequences
(see, \eg \cite{mancini-etal:2013:cav,mancini-etal:2015:sylvaas-pdp}).
To find an optimal treatment means to find an optimal plan in hybrid domains, where the behaviour of the given
system is described by both discrete and continuous quantities.
%
In the literature, there are many techniques to model planning problems in
hybrid domains,
\eg PDDL+ \cite{fox-etal:2006:jair,vallati-etal:2016:aaai}.
Most of PDDL+ planners can deal only with linear dynamics
(\eg \cite{coles-etal:2014:icaps}).
\cite{bryce-etal:2015:aaai} proposed
a \Ac{SMT}-based approach for solving PDDL+ problems with non-linear dynamics.
Model checking techniques are also used to find plans. Examples in this
direction are \cite{bogomolov-etal:2014:aaai,bogomolov-etal:2015:icaps},
which exploits symbolic model checking,
UPMurphi \cite{dellapenna-etal:2009:icaps,dellapenna-etal:2010:planning}, which given as input a PDDL+
problem specification computes a universal plan, CGMurphi~
\cite{dellapenna-etal:2013:eurjcontrol}, an explicit model checker used to
compute optimal controllers,
and \cite{alimguzhin-etal:2017:tac,mari-etal:2014:tosem,mazo-etal:2010:cav,rungger-etal:2016:hscc},
which define methodologies to compute
controllers for non-linear hybrid systems.
However, as outlined in \cref{sec:computing:simulation}, the typical complexity of the differential equations of \Ac{VPH} models
relevant for clinical practice makes such models out of reach for
symbolic approaches like those mentioned above, and appoints numerical integration as the only viable means to compute (black-box) the model evolutions under a given input function.

In particular, even considering that clinical actions have constant and equal duration (as, \eg in \cite{li-etal:2008:icaps}), no reasoning or inference can be made on action effects in a black-box setting as ours, because the only way to interact with the models is through numerical simulation.

The automated synthesis of rational decisions and plans in black-box environments is common in several other application domains of high industrial relevance, like smart grids (see, \eg
\cite{mancini-etal:2014:smartgridcomm,mancini-etal:2015:dsd,hayes-etal:2016:tsg}), games (see, \eg \cite{lipovetzky-etal:2015:ijcai}) and real-time manoeuvring of \Acl{UAV} (see, \eg \cite{ramirez-etal:2017:ijcai}).

The works closest to ours are those in~\cite{lipovetzky-etal:2015:ijcai,frances-etal:2017:ijcai} and citations thereof, where a simulator is used to discover the effect of actions.
In such works, the simulator is defined as a factored state model where actions are (black-box) procedures and states are represented in terms of variables.
Then an algorithm, namely, Iterated Width ($\Fun{IW}$), is typically employed.
%
It consists of iteratively calling a breadth-first procedure, namely, $\Fun{IW}(i)$, with $i=1, 2, 3, \ldots$, until the problem is solved or $i$ becomes greater than the number of state variables (see, \eg \cite{lipovetzky-etal:2012:ecai}).
%
During each call to $\Fun{IW}(i)$,
states are pruned accordingly to how novel they are.
A state is novel if and only if values for at most $i$ state variables have not seen before.
%
Authors point out that $\Fun{IW}$ is efficient for the majority of classical planning problems where it is enough that $i=1,2$, \ie actions change at most 2 state variables. 
However, in our setting, our simulator state consists of the union of all state vectors, \ie $\Vec{x}(t)$, of each \Ac{VP}{+}monitor within the input \digitaltwin.
%
Moreover, the most of variables within such state vectors consist of real-valued biological quantities.
Also, we remind that the dynamics of such model are defined by means of \Acp{ODE}.
%
Hence, when we apply a clinical action (and simulate our \digitaltwin) the vast majority of state variables change their value. In this setting, applying $\Fun{IW}$ means nearly always to call only $\Fun{IW}(n)$, with $n$ the overall number of variable of our simulator state. 
% 
This behaviour makes the pruning on which $\Fun{IW}$ relies on quite ineffective as $\Fun{IW}$ degenerates to prune truly duplicate states, which are also extremely rare as our variables are real valued.
%
Note that, in order to increase pruning of duplicate states, one could think of simplifying the dynamics of the \Ac{VPH} model at hand (\eg by discretising state variable domains).
%
However, this is not a straightforward approach as it poses several questions about accuracy, credibility, and trust of the entailed model predictions, which have to be again experimentally assessed.


==> 03.preliminaries/clinical-records.tex <==
%!TEX root = ../root.tex
In order to compute personalised optimal treatments, we will start from clinical data collected from a human patient.
Along the lines of \cite{mancini-etal:2014:fmcad}, a clinical record \CR{C} (\cref{def:clinical-record}) consists of a sequence of measurements for all biological quantities of interest, where each measurement maps a time instant to a measured value.

\begin{definition}[Clinical record]
\label{def:clinical-record}
Let $S_1, \ldots, S_p$ be the biological quantities of interest.
A patient clinical record, \CR{C}, is a tuple $(C_1, \dots, C_p)$, where each $C_i$ ($i \in [p]$) is a finite sequence of pairs $(t, v)$ (possibly empty) where $t \in \RealsGEZ$ denotes a time instant and $v \in \RealsGEZ$ is the measured value of biological quantity $S_i$.
\end{definition}

In our case study (fertility treatments), clinical records of interest collect measurements for the main hormones involved in the human menstrual cycle, namely: \Ac{LH}, \Ac{FSH}, \Ac{E2}, and \Ac{P4}.

==> 03.preliminaries/content.tex <==
%!TEX root = ../root.tex
In this section we give the necessary background knowledge.
We denote with \Reals, \RealsGEZ, \RealsGZ, \IntegersGEZ, and \IntegersGZ 
the sets of, \respectively, all real, non-negative real, strictly positive real, non negative, and strictly positive integer numbers.
Given $n \in \IntegersGZ$, we denote by $[n]$ the set of integers $\Set{1, \ldots, n}$.

\subsection{\Acl{VPH} models}
\label{sec:computing:model}
\Input{vph.tex}

\subsection{The GynCycle \Acl{VPH} model}
\label{sec:preliminaries:gyncycle}
\Input{gyncycle.tex}


\subsection{GynCycle \Aclp{VP}}
\label{sec:preliminaries:vp}
\Input{vp.tex}


\subsection{Clinical records}
\label{sec:data}
\Input{clinical-records.tex}



\subsection{Digital twin of a human patient}
\label{sec:digital-twin}
\Input{digital-twin.tex}

==> 03.preliminaries/digital-twin.tex <==
%!TEX root = ../root.tex
To compute a personalised treatment for a human patient, we first need to compute a \emph{digital representation} for her.
%
This will be done by using clinical data (in the form of a clinical record $\CR{C}$, \cref{def:clinical-record}) available from that patient in order to select, from our representative population of \Acp{VP}, the subset of \Acp{VP} that are \emph{compatible} with (\ie fit) such data.

To do so, we proceed as follows.
Let \CR{C} be a clinical record and $\lambda$ be a \Ac{VP} of our population.
We define $\MAPE{\CR{C}}{\lambda}$ as the average (over all biological quantities $S_i$, $i \in [p]$) \Ac{MAPE} between the clinical measurements of $S_i$ in \CR{C} and time evolutions of $S_i$ in \Ac{VP} $\lambda$.
Formally:
\begin{equation*}
\MAPE{\CR{C}}{\lambda} ~=~
	\frac{1}{p} \sum_{i=1}^{p} 
		\frac{1}{\SetCardinality{C_i}} 
			\sum_{(t, v_i) \in C_i} 
				\Abs{ 
					\frac
						{v_i - x_i(\lambda, t)}
						{\zeta(v_i)}
				}
\end{equation*}
%
where $\zeta(v_i)$ is $v_i$ if $v_i \neq 0$ and a small positive constant otherwise (to avoid division by zero).

By using such a metric, \cref{def:digitaltwin} defines the concept of \emph{patient \digitaltwin} as the set of \emph{all} \Acp{VP} $\lambda$ in our population $\Pop$ having a value for $\MAPE{\CR{C}}{\lambda}$ up to a given threshold. 

\begin{definition}
\label{def:digitaltwin}
	Given a clinical record \CR{C}, %$\mathcal{L}$, 
	our complete population of \Acp{VP} $\Pop$, 
	a threshold $\delta \in \RealsGEZ$ for our error metric $\MAPE{}{}$, the \emph{digital twin} $P$ of \CR{C} is the following set:

	\begin{equation*}
		\DT{\CR{C}} = \Set{ 
			\lambda \in \Pop ~\middle|~  
				\MAPE{\CR{C}}{\lambda} \leq \delta 
		}.
	\end{equation*}
\end{definition}

Intuitively, the \digitaltwin of a human patient is a \emph{digital} representation of the patient physiology in the form of \emph{all} \Acp{VP} entailing model behaviours that fit the patient clinical measurements (up to an average \Ac{MAPE} $\delta$).

==> 03.preliminaries/equations.tex <==
\begin{align*}
\dot{\LH}_\blood(t) &= \frac{\LH_\pit(t)}{V_\blood}\cdot \left(b^{\LH}_\Rel + k_\GR^\LH\cdot H^+(\GR(t),T_\GR^\LH;n_\GR^\LH) \right)\\
                    &- (k_\on^\LH \cdot \R_\LH (t) +k_\cl^\LH) \cdot \LH_\blood (t) \notag\\
\dot{\FSH}_{\blood} (t) &=  \frac{\FSH_\pit(t)}{V_\blood}\cdot \left(b^{\FSH}_\Rel + k_\GR^\FSH\cdot H^+(\GR(t),T_\GR^\FSH;n_\GR^\FSH)\right)\\
                        &- ( k_\on^\FSH\cdot \R_\FSH(t) + k_\cl^\FSH)\cdot\FSH_\blood(t) \notag\\
% \dot{\E2}(t) &= b^\E2 + k_{\AFb}^{\E2}\cdot{\AFb}(t) + k_\AFc^\E2 \cdot \LH
% (t)\cdot\AFc(t)\\ 
%             & + k_\AFd^\E2 \cdot\AFd(t) \quad + k_\PrF^\E2 \cdot\LH
% (t)\cdot\text{PrF}\\
%             & + k_\Luta^\E2\cdot\Luta(t) + k_\Lutd^\E2\cdot\Lutd(t)-k_\cl^\E2\cdot\E2(t)\notag\\
% \dot{\P4}(t) &= b^\P4+k_\Lutd^\P4\cdot\Lutd(t)-k_\cl^\P4\cdot\P4(t) \notag\\
\end{align*}


==> 03.preliminaries/gyncycle.tex <==
%!TEX root = ../root.tex

%\Ac{VPH} models are mechanistic models of the human physiology (focussing the whole body or on selected compartments), providing quantitative information about time evolutions of biological species or substances of interest. 

\Comment{
In this section we describe the GynCycle \Ac{VPH} model, presented and validated in~\cite{roeblitz-etal:2013:theorbio}, which we will use as our case study.
}
In this section we describe the GynCycle \Ac{VPH} model, presented and evaluated in~\cite{roeblitz-etal:2013:theorbio}, which we will use as our case study. 

%
GynCycle is an \Ac{ODE}-based model of the human female \Ac{HPG} axis, with a special focus on the interactions and feedback mechanisms between hormones like \Ac{GnRH}, \Ac{FSH}, \Ac{LH}, \Ac{E2}, \Ac{P4}, \Ac{IhA}, and \Ac{IhB} during the different stages of the menstrual cycle.
  
The model defines the time evolution of overall $33$ biological quantities (mostly blood concentration of hormones) and the \Ac{PKPD} of several pharmaceutical drugs used in assisted reproduction (in particular, we will focus on \Ac{GnRH} analogues like Triptorelin) %, or \Ac{FSH}/\Ac{LH}--based drugs) 
by means of highly non-linear differential equations.

For example, equations defining the time evolution of \Ac{LH},
and \Ac{FSH}
% , \Ac{E2} and \Ac{P4}
are as follows:

\Input{equations.tex}

In the differential equations above, $\LH(t)$, $\FSH(t)$ etc.\ denote biological \emph{species} of interest (in the example, the blood concentration of \Ac{LH} and \Ac{FSH}, \respectively), while
$b^\LH_\Rel$, $k^\LH_\cl$, etc.\ denote \emph{model parameters}.

As such, GynCycle is a \emph{hybrid system} whose inputs represent drug administrations.
%
As it happens with \Ac{VPH} models of practical interest as GynCycle, the number and complexity of their differential equations makes symbolic analysis (by, \eg a model checker for hybrid systems) an unviable option. 
%
Indeed, the model can be \emph{simulated} by means of numerical integration in order to compute the time evolution of the hormones of interest upon administration of a sequence of drug doses. 
%
Thus, GynCycle is used as an \emph{executable} black-box model. 




==> 03.preliminaries/vp.tex <==
%!TEX root = ../root.tex
\Ac{VPH} models like GynCycle typically take into account inter-subject variability (\ie the physiological differences among different individuals) by including suitable \emph{parameters} in their equations (like $b^\LH_\Rel$ and $k^\LH_\cl$ mentioned above).
Different value assignments to model parameters yield different model time evolutions and/or different reactions to drug administrations, thus defining different \Acp{VP}.
Intuitively, each \Ac{VP} represents a class of indistinguishable (as long as the \Ac{VPH} model is concerned) patients.
%
Computing a complete set of \Acp{VP} for the model at hand is the starting point to obtain a \emph{representative} population of virtual patients (hence, ideally showing all possible phenotypes). In turn, this is the key enabler to perform \Acp{ISCT} to assess, \eg safety and/or efficacy of a pharmacological treatment.

% Unfortunately, computing the complete set of \Acp{VP} defined by a complex \Ac{VPH} model is all but easy.
% In fact, arbitrarily setting single model parameters independently (although to values belonging to their legal bounds) very often results in overall model trajectories that are \emph{physiologically meaningless}, \ie that do not represent behaviours that are physiologically possible in humans. 
% %
% This is because many constraints often exist among such parameters, which however, are not explicitly defined in model (mainly because of lack of precise physiological knowledge).
% %
% Also, although many parameters define physical quantities (\eg the rate of secretion of a given hormone by a gland), parameters are also introduced to enable modelling shortcuts, in order to abstract away not-well-understood physiological mechanisms. All this results in \Ac{VPH} models which are greatly over-parametrised, with hidden dependencies among parameters that make the search for a complete population of \Acp{VP} extremely challenging.

% For example, the GynCycle model defines 75 (real-valued) parameters, whose values are patient-specific. Even if we discretise the (continuous) domain for each parameter in only 10 values (hence, assuming that a variation of 10\% of each value will not yield a major impact of physiological behaviour), the size of the search space of possible \Acp{VP} would be $10^{75}$. By considering that numeric simulation of the differential equation--based model is needed to assess the physiological meaningfulness of each prospective \Ac{VP}, all this makes any hope for exhaustive search vain. 
% %
% Also, because of the many mechanisms occurring in the \Ac{HPG} axis not precisely known at a fine-grain level (and hence, not modelled), the model is greatly over-parametrised and only a few combinations of values to such parameters do actually yield physiologically meaningful model trajectories.
% Hence, a naive random sampling of the search space will produce (with very high probability) very few physiologically meaningful \Acp{VP} (if any at all), even after billions of tries.

% To overcome this problem, in~\cite{mancini-etal:2014:fmcad} we have exploited a statistical model checking--based approach using a non-uniform sampling process finely tuned against the model. Our algorithm can be massively parallelised on large \Ac{HPC} infrastructures~\cite{mancini-etal:2015:iwbbio} in order to compute, once and forall, a population of \Acp{VP} for a \Ac{VPH} model. The population is complete \wrt to the used sampler up to an arbitrarily high statistical confidence. After running our algorithm on the GynCycle model with reasonable values for the target statistical confidence on completeness, we generated a representative population of \Acp{VP} consisting of the order of $10^4$ individuals (out of $10^{75}$ possible parameter assignments).

% Such a population will be the starting point of our \Ac{ISCT}.


Unfortunately, computing the complete set of \Acp{VP} defined by a complex \Ac{VPH} model like GynCycle is all but easy from the computational point of view, and may require weeks of massive simulation on large \Ac{HPC} infrastructures.
%
This is due to the hidden presence of inter-dependency constraints among elements of the parameter vector which are usually not explicitly known, and hence not modelled. %cannot be taken into account constructively. 
By ignoring such constraints (which would happen by, \eg choosing values for the parameter vector elements in a uninformed random way) would yield with high probability to model behaviours that violate the laws of biology (and hence such parameter assignments could not be regarded as \Acp{VP}).

In~\cite{mancini-etal:2014:fmcad,mancini-etal:2015:iwbbio}, a statistical model checking--based approach using intelligent global search heuristics has been discussed. 
Such a methodology enables the computation of a population of \Acp{VP} (parameter assignments showing time evolutions compatible with the laws of biology) that is complete \wrt the used heuristics up to an arbitrarily high statistical confidence. 
%
This approach was recently generalised in \cite{calabrese-etal:2019:rcra}, where it proved its effectiveness in computing a population of \Acp{VP} for a \Ac{VPH} model of the glucose regulation system in patients with Type 1 Diabetes Mellitus.

In this paper, we conduct our \Acp{ISCT} starting from a population $\Pop$ of around $\DataGet{exps/results/population}$ \Acp{VP}, extracted using the algorithm in \cite{mancini-etal:2014:fmcad,mancini-etal:2015:iwbbio} from a huge search space of \Pretty{e75} possible candidate parameter vector assignments (set $\Lambda$ in \cref{def:vph-formalisation}). 
By exploiting \emph{model locality} assumptions typically made on \Ac{ODE}-based \Ac{VPH} models (\ie small changes in the model parameters are expected to yield small changes in the overall model trajectory), the domain of each of the \Pretty{75} dimensions of $\Lambda$ has been discretised into \Pretty{10} possible values (see \cite{mancini-etal:2014:fmcad} for an evaluation of the appropriateness of this choice).
%
We then ran the parallel tool described in \cite{mancini-etal:2015:iwbbio} with error threshold equal to \Pretty{0.01}\% and statistical confidence bound equal to \Pretty{95}\%.
This means that, upon termination, we have \Pretty{95}\% confidence that the probability of finding new \Acp{VP} by further searching is at most \Pretty{0.01}\%.



==> 03.preliminaries/vph.tex <==
%!TEX root = ../root.tex
\Ac{VPH} models usually are \emph{hybrid systems}
defined by means of \Acp{ODE} (see, \eg \cite{sontag:1998:book,alur-etal:2001:hscc,bartocci-etal:2016:plos-comp-bio,wang-etal:2016:hldvt}) as stated in \cref{def:vph-formalisation}.

\begin{definition}
\label{def:vph-formalisation}
\AcronymReset{ODE}%
A parametric \Ac{ODE} dynamical system is defined by a set of differential equations over time (variable $t \in \RealsGEZ$) having the following form:
\begin{equation*}
  \dot{\Vec{x}}(t) = \Vec{f}(\Vec{x}(t), \Vec{u}(t), \lambda)
\end{equation*}
where:
	\begin{itemize}
	  \item $\Vec{x}(t) \in \Reals^{n_x}$ is called \emph{state vector}, and models biological quantities;
	  \item $\Vec{u}(t) \in \Reals^{n_u}$ is called \emph{input vector}, and models exogenous inputs (\eg sequences of drug administrations);
	  \item $\Lambda \subseteq \Reals^{n_\lambda}$ is called \emph{parameter space} and $\lambda \in \Lambda$ denotes a \emph{parameter vector};
	  \item $\Vec{f}$ is a vector of functions defining system dynamics.
	\end{itemize}
	Above, we have $n_x, n_u, n_\lambda \in \IntegersGZ$.
	% of the vectors above are positive integers.
\end{definition}

In our setting, \emph{administrations of $n_u$ different pharmaceutical drugs} (clinical actions) define inputs to the \Ac{VPH} model.
%
Indeed, for each $i \in [n_u]$, the $i$-th component $u_i$ of the input vector $\Vec{u}$ defines a function that associates to each time instant $t \in \RealsGEZ$ the administered dose of the $i$-th drug, to be chosen within a set $A_i$ of possible doses (which always includes dose zero).

Given an assignment $\lambda$ to the \Ac{VPH} model parameters and an input vector $\Vec{u}$ (\ie a time sequence of administrations of the $n_u$ drugs defined within the model), the associated \Ac{VPH} \emph{model trajectory} is a continuous-time function $\Vec{x}_\lambda(t)$ (or, to simplify notation, $\Vec{x}(\lambda, t)$)
representing the time evolution of the biological quantities defined by the model when fed with $\Vec{u}$ starting from its initial state and with its parameters set to $\lambda$.
Of course, as the \Ac{VPH} model is causal, its trajectories up to any time point $\overline{t} \in \RealsGEZ$ only depend on the \emph{restriction} of the input up to time point $\overline{t}$ (see, \eg \cite{sontag:1998:book,mancini-etal:2017:ipl}).

==> 04.treatment/content.tex <==
%!TEX root = ../root.tex
In this section we define the treatment we used as our case study: the downregulation phase of an assisted reproduction protocol currently administered at the Department of Reproductive Endocrinology of University Hospital Zurich.

At each menstrual cycle of a human female, among the several follicles initially present in the ovaries, only one, unless in exceptional cases, grows and reaches maturity. 
A complex competition among follicles takes place, driven by a hormone-based feedback loop, in order to inhibit the maturation of multiple follicles. 


An assisted reproduction treatment aims at neutralising (through drugs) such a feedback loop (\emph{downregulation phase}), in order to achieve a controlled and an
as-simultaneous-as-possible growth of \Pretty{5}--\Pretty{15} ovarian follicles (\emph{stimulation
phase}). 
When the first three follicles reach a size where a mature oocyte (\ie an egg cell ready for fertilisation) can be expected (about \Pretty{18}~mm in diameter), ovulation is induced. Then, the oocytes are retrieved, those which are mature are tried to be fertilised \emph{in vitro}, and implanted either immediately within the treatment cycle or later after cryopreservation (\ie a preservation process by cooling) back into the uterus.

Assisted reproduction treatments are complex and challenging, with low average success rates (around \Pretty{30}\%) even in the top clinics, and with many factors that, to date, can be hardly kept under full control. 
Indeed, as hormonal regulatory systems occur within a complex network of endocrinological, neurological and psychological factors \cite{leeners-etal:2017:behavioral,hengartner-etal:2017:psycho,leeners-etal:2019:front-psychol}, they are difficult to capture within clinical studies, and model-based approaches might be of great aid in taking these many factors under better control.

Our case study is one of the worldwide classically used downregulation protocols
aiming at suppressing the usual hormonal oscillations of the menstrual cycle (as in \cref{fig:downregulation}) and preparing the patient to the
following stimulation. 

\begin{figure}
	\centering
	%
	\hfill
	\begin{subfigure}{\DataGet{paper/figures/subfigures/cols/2/width}}
		\IncludeGraphics
			[width=\linewidth]
			{figures/downregulation-expected-E2.pdf}
			%
			\caption{\Acs{E2}}
	\end{subfigure}
	\hfill
	\begin{subfigure}{\DataGet{paper/figures/subfigures/cols/2/width}}
		\IncludeGraphics
			[width=\linewidth]
			{figures/downregulation-expected-P4.pdf}
			%
			\caption{\Acs{P4}}
	\end{subfigure}
	\hfill
	
	\hfill
	\begin{subfigure}{\DataGet{paper/figures/subfigures/cols/2/width}}
		\IncludeGraphics
			[width=\linewidth]
			{figures/downregulation-expected-FSH.pdf}
			%
			\caption{\Acs{FSH}}
	\end{subfigure}
	\hfill
	\begin{subfigure}{\DataGet{paper/figures/subfigures/cols/2/width}}
		\IncludeGraphics
			[width=\linewidth]
			{figures/downregulation-expected-LH.pdf}
			%
			\caption{\Acs{LH}}
	\end{subfigure}
	\hfill

	
	\caption{Expected downregulation effects on some of the hormones playing a role in the human female menstrual cycle. The coloured area defines the time window during which Triptorelin is administered.}
	\label{fig:downregulation}
\end{figure}

At the Department of Reproductive Endocrinology of University Hospital Zurich, this protocol currently consists of a sequence of daily administrations of \Pretty{0.1}~mg of Triptorelin, a \Ac{GnRH} analogue. 
For physiological reasons, downregulation is started within a precise time
window of the menstrual cycle, namely between day 
\DataGet{exps/treatment day min start} and day 
\DataGet{exps/treatment day max start}.
%
The treatment might have different duration in order to address different
patient reactions. 
In particular, a downregulation treatment is considered \emph{successful}
(effective) for a patient in case the blood concentrations of a given set of
hormones and other physiological quantities go below certain thresholds within 9 days from the first drug administration, and stay always below such thresholds for the following \Pretty{21} days. 
As a consequence, a downregulation treatment might last up to \Pretty{30} days.


==> 05.treatment-design/algo/action-ordering.tex <==
%!TEX root = ../../root.tex
In a black-box setting as ours, no inference can be made on the effects of each candidate action without performing a simulator run to actually advance the model and then querying the model monitor output.
%
Hence, approaches to compute, through inference, a dynamic preference order among the candidate actions to be tried during search (as those exploited in, \eg classical planning, planning for white-box hybrid systems --see \cref{sec:state-of-the-art}-- or (Q)CSP, SAT or local search solvers, see \eg \cite{rossi-etal:2006:constraint,biere-etal:2009:sat,glover-etal:2006:metaheuristics,gottlob-etal:2007:conditional,mancini-etal:2008:constraints,bordeaux-etal:2008:jair,bordeaux-etal:2009:tocl}) cannot be applied.

The only information available to the algorithm without running the simulator is value $D_\text{min}$ and the overall cost of the \emph{current} partial treatment (overall amount of drug administered).
Hence, given that our algorithm searches for a successful treatment of minimum cost and that any action has a non-negative contribution to the overall treatment cost, not surprisingly tries the clinical actions on each node in the search tree in ascending order of their associated dose (\ie cost), hence performing a \emph{greedy}, optimistic choice.


==> 05.treatment-design/algo/content.tex <==
%!TEX root = ../../root.tex
%
In this section we describe our intelligent search that drives a \digitaltwin simulator, by defining our
search tree (\cref{sec:search:tree}) and criteria for the evaluation and expansion of search tree nodes (\cref{sec:safety}).
We also introduce two ordering heuristics aiming at efficiently pruning the search tree (\cref{sec:action:order}) and speeding up the \digitaltwin simulation time (\cref{sec:order:vp}), while retaining completeness of the overall algorithm.

\subsubsection{Search tree definition}
\label{sec:search:tree}
\Input{tree.tex}

\subsubsection{Search tree node evaluation and expansion}
\label{sec:safety}
\Input{safety-goal.tex}

\subsubsection{Optimality constraint}
\label{sec:optimality}
\Input{optimality.tex}

\subsubsection{Action ordering heuristic}
\label{sec:action:order}
\Input{action-ordering.tex}

\subsubsection{Dynamic \Acs{VP} simulation ordering}
\label{sec:order:vp}
\Input{vp-ordering.tex}


==> 05.treatment-design/algo/optimality.tex <==
%!TEX root = ../../root.tex
Since we seek the \emph{optimal} personalised treatment for the input \digitaltwin,
our algorithm does not stop at the first found successful treatment.
Indeed, along the lines of \cite{mancini-etal:2012:sac}, it keeps track of the \emph{lightest} successful treatment found so far, \ie the one envisioning the administration of the \emph{minimum} overall drug amount $D_\text{min} \in \RealsGEZ$.
Initially, $D_\text{min}$ is set to $+\infty$. 

At each node of the search tree, any action extending the current partial treatment with an administration of a drug dose which would make the overall administered drug amount reaching or exceeding $D_\text{min}$ is regarded as not applicable.

The optimality constraint (whose threshold is updated each time a new optimal treatment is found), the presence of a bounded horizon $h$ and the fact that our algorithm does not stop at the first successful treatment clearly guarantee that a global optimum is always returned (if any successful treatment exists).


==> 05.treatment-design/algo/safety-goal.tex <==
%!TEX root = ../../root.tex
%
At each node of the search tree, our algorithm needs to extend the current sequence of clinical actions (a treatment \emph{prefix}, which is the empty sequence in the initial state).
To do so, the algorithm:
\begin{enumerate}
	\item Stores the current states of the \Ac{VP} models by means of a $\Fun{store}$ command.
	\item For each clinical action $a \in A_1 \times \ldots \times A_{n_u}$ (according to the heuristic ordering discussed in \cref{sec:action:order}), injects $a$ into the simulator and advances the simulation (simultaneously for all \Acp{VP} defined within the simulator) by time $\tau$ (this is done by issuing a command $\Fun{run}(a,\tau)$).
	\item If the monitor output for one \Ac{VP} returns \Unsafe, the algorithm infers that there is no hope to extend the partial treatment to a complete treatment successful for all the \Acp{VP} in the \digitaltwin and issues a backtrack, by loading back (via a $\Fun{load}$ command) the simulator state of all \Acp{VP} associated to the parent node in the search tree.
	\item \label{step:solution} Otherwise, if the monitor output for all \Acp{VP} is \Success, the algorithm infers that the current treatment is successful for all \Acp{VP}.
	\item Otherwise, the algorithm continues by expanding the new search tree node and extending the current treatment prefix.	
\end{enumerate}	

Whenever no further actions can be executed in the current node of the search tree, the current simulator state is freed from memory by a $\Fun{free}$ command before triggering a backtrack.

In order to reduce the required simulation time when expanding each node, the multiple model copies are not actually packaged into a single (much heavier to be simulated) model, but are kept separate and simulated \emph{sequentially}.
This allows our algorithm to perform two performance optimisations: a sort of \emph{early pruning} of the current treatment prefix %on the different \Acp{VP} 
and a \emph{dynamic revision of the order} with which the \Acp{VP} in the input \digitaltwin will be actually simulated in the sequel (\cref{sec:order:vp}).


==> 05.treatment-design/algo/tree.tex <==
%!TEX root = ../../root.tex
Given a patient clinical record \CR{C}, its \digitaltwin \DT{\CR{C}}, and possible alternative doses for each treatment drug at hand (\ie sets $A_1, \ldots, A_{n_u}$, each one including dose zero), our backtracking-based algorithm performs a search in the space of possible treatments (\ie time sequences of clinical actions in $A_1 \times \cdots \times A_{n_u}$).
%
Under the following assumptions: 
(i)~the sets of allowed doses $A_1, \ldots, A_{n_u}$ for the $n_u$ drugs are \emph{finite};
(ii)~drug administrations occur at time instants multiple of a given \emph{time-quantum} $\tau \in \RealsGZ$;
and (iii)~sought treatments have a bounded duration ($\tau h$, with $h \in \IntegersGZ$ being the treatment \emph{horizon}),
% 
we can limit our search to a \emph{finite tree} of maximum depth $h$, 
where each tree node at depth $0 \leq l \leq h$ defines a \emph{discrete sequence} of $l$ clinical actions
(elements of $A_1, \ldots, A_{n_u}$), each one occurring in the first $l$ time points multiple of $\tau$.

As described in \cref{sec:computing:simulation}, our search algorithm drives a simulator containing multiple copies of the \Ac{VPH} model (one per \Ac{VP} in the \digitaltwin given as input), each one connected to a copy of the monitor which checks for treatment invariants and goals.

Accordingly, each node of our search tree keeps also track of the \digitaltwin simulator state reached by injecting the clinical action sequence of that node.
This is done via a $\Fun{store}$ command (see \cref{sec:computing:simulation}).
A transition between a parent node and a child node 
consists of extending the clinical action sequence of the parent node with a new action $a \in A_1 \times \cdots \times A_{n_u}$. In doing so, we also advance the \digitaltwin simulator state of the parent node via a $\Fun{run}$ command (see \cref{sec:computing:simulation}).
In \cref{sec:safety}, we describe more in details how a search tree node is evaluated and expanded. 

Before the search starts, for each \Ac{VP} $\lambda$ in the input \digitaltwin, we prepare its associated copy of the \Ac{VPH}{+}monitor model within the \digitaltwin simulator, by setting the parameter vector to $\lambda$.
We also store the initial simulator state via a $\Fun{store}$ command (see \cref{sec:computing:simulation}). 

Clearly, the assumptions above together with the entailed search tree structure hold for a very wide class of treatments.
%
For example, in our downregulation treatment case study, there is only one possible drug, namely Triptorelin, hence $n_u = \Pretty{1}$. 
Also, as such treatments allow at most one Triptorelin administration per day, we can safely set $\tau = \text{1 day}$.
Finally, successful treatments cannot last more than 
	$h = \Pretty{25}+\Pretty{9}+\Pretty{21} = \Pretty{55}$ days, 
starting from day \Pretty{1} of the patient menstrual cycle (\ie the latest cycle day, \Pretty{25}, when the treatment might start, plus the latest day, 9, within which the safety conditions must be met, plus the number of consecutive days, \Pretty{21}, in which the safety conditions must be always satisfied in order to declare success). 

Moreover, in our case study, the initial simulator state represents day \Pretty{1} of the menstrual cycle of all \Acp{VP} in the input \digitaltwin. 


==> 05.treatment-design/algo/vp-ordering.tex <==
%!TEX root = ../../root.tex
%
When, during the evaluation of search tree node, the monitor output after the simulation of a \Ac{VP} in the \digitaltwin returns \Unsafe, our algorithm, by performing a sort of \emph{early pruning}, does not simulate nor evaluate the remaining \Acp{VP}, but it backtracks and tries the next available action from the parent node, if any. 
%
Upon backtracking, the algorithm changes the verification ordering of the \Acp{VP} in the \digitaltwin in such a way that those \Acp{VP} not satisfying treatment invariants or not yet simulated in the previous search step are simulated \emph{first}. 
%
The rationale is that those \Acp{VP} that already satisfied treatment invariants in previous step, will more likely satisfy treatment invariants in the current step, where a slightly different drug dose is chosen.


==> 05.treatment-design/content.tex <==
%!TEX root = ../root.tex
%
In this section, we define the conditions of a successful treatment through invariants and goals (\cref{sec:computing:monitor}), describe how to perform \digitaltwin simulations (\cref{sec:computing:simulation}), 
and describe the algorithm used at the core of our optimal personalised treatment computation (\cref{sec:search}).

\subsection{Modelling treatment invariants and goals}
\label{sec:computing:monitor}
\Input{monitors.tex}


\subsection{\DigitalTwin simulation}
\label{sec:computing:simulation}
\Input{simulation.tex}


\subsection{Intelligent backtracking--driven simulation}
\label{sec:search}
\Input[algo]{content.tex}


==> 05.treatment-design/figures/monitor.tex <==
%!TEX root = ../../root.tex
\def\tmpScale{0.5}

\usetikzlibrary{positioning}
\usetikzlibrary{calc}
\usetikzlibrary{decorations.pathmorphing}

\begin{tikzpicture}[
      semithick,->,
      %scale=\tmpScale, 
      %every node/.style={scale=\tmpScale},      
      node distance=3cm
]
            \tikzstyle{final state} = [state, double] %[fill=lightgray]
            \tikzstyle{state} = [rounded corners]
            
            \node[draw,state] (safe) {\Safe};   
            \node[final state,draw,right = of safe] (unsafe) {\Unsafe};            
            \node[final state,draw,right = of unsafe] (success) {\Success};

            %\path (start) edge (safe);
            \draw [->,decorate,decoration={snake, amplitude=.4mm}] 
                  ($(safe) - (1.5cm, 0cm)$) -- (safe);

            \path (safe) edge node[above] {invariants violated} (unsafe);
            \path (safe) edge [bend right=15] node[below] {goal reached} (success);

\end{tikzpicture}
      

==> 05.treatment-design/monitors.tex <==
%!TEX root = ../root.tex
We define conditions that must be \emph{always} and \emph{eventually} satisfied by a successful treatment by means of \emph{invariants} and \emph{goals}, \respectively.
%
Invariant and goal treatment conditions are modelled as continuous-time \emph{monitors} embedded within the \Ac{VPH} model, along the lines of \cite{mancini-etal:2013:cav,mancini-etal:2016:micpro}.
Monitors observe the state of the system and check whether the properties of interest are satisfied. 

In particular, given a model trajectory $\Vec{x}(\lambda, t)$ under a given input $\Vec{u}$, our monitor output is \Safe as long as $\Vec{x}(\lambda, t)$ satisfies the invariants (in other words, the monitor decision is ``undetermined'' as long as there is \emph{hope} to extend the current treatment into a successful treatment) and goes to and \emph{stays} at value \Unsafe as soon as invariants are \emph{violated}. 
%
When a \Safe model trajectory satisfies the goal conditions, the monitor output turns to \Success, informing the caller that the input $\Vec{u}(t)$ defines a \emph{successful} treatment (\ie an \emph{effective} treatment which \emph{always} satisfies invariants). 

The use of continuous-time monitors embedded in the \Ac{VPH} model gives us a flexible way to model both bounded safety and bounded liveness properties, and is a standard approach in the simulation-based verification of cyber-physical systems (see, \eg \cite{mancini-etal:2014:dsd-anytime,mancini-etal:2015:sylvaas-pdp}).

In our case study, the properties of interest are the conditions of successful downregulation treatments (\cref{sec:treatment}). 
%
In particular, our \emph{invariant} requires that the day of the first drug administration is between day \Pretty{21} and day \Pretty{25} of the menstrual cycle. 
Moreover, the value of all the biological quantities under observation must go and stay below their thresholds from the \Pretty{9}-th day after the first drug administration. Our \emph{goal condition} instead requires that values for those quantities stay below their thresholds for \Pretty{21} consecutive days.

As a consequence, our monitor output is \Safe in the initial state, and eventually turns either to \Unsafe or to \Success (see \cref{fig:monitor}). Model output turns to value \Unsafe as soon as, from the \Pretty{9}-th day after the first drug administration, the value of \emph{any} of the physiological quantities under observation exceeds its threshold. Conversely, model output turns from value \Safe to value \Success as soon as all the thresholds are satisfied for \Pretty{21} consecutive days. 

\begin{figure}
	\centering
    \Input{figures/monitor.tex}
    \caption{Treatment monitor.}
    \label{fig:monitor}
\end{figure}

==> 05.treatment-design/simulation.tex <==
%!TEX root = ../root.tex
As anticipated in \cref{sec:preliminaries}, the complexity of the (highly non-linear) differential equations typically occurring in actual \Ac{VPH} models hinders the possibility for their symbolic analysis. 
Numerical \emph{simulation} is often the only means to compute the time evolution of the model quantities of interests (mainly blood hormone concentrations in our case study GynCycle model) upon a sequence of clinical actions (administration of one or more drugs with their associated doses). Also, as \Ac{VPH} model equations are often stiff, simulation can be an \emph{expensive} process from a computational point of view.

Our algorithm for optimal personalised treatment computation regards the input \Ac{VPH} model as an \emph{executable} black-box model. 
%
In order to drive the \Ac{VPH} model simulator, our algorithm assumes that it accepts the following basic commands (which are available or can be readily implemented within most modern simulators~\cite{mancini-etal:2014:pdp,mancini-etal:2016:fundam}):
$\Fun{store}$, $\Fun{load}$, $\Fun{free}$, $\Fun{run}$, $\Fun{get}$.
Command $\Fun{store}(l)$ stores in memory the current state of the simulator and labels with $l$ such a state.
Command $\Fun{load}(l)$ loads into the simulator the stored state labelled with $l$.
Command $\Fun{free}(l)$ removes from the memory the state labelled with $l$.
Command $\Fun{run}(a, t)$ (with $a \in A_1 \times \cdots \times A_{n_u}$ and $t \in \RealsGZ$) executes clinical action $a$ (thus administering given --possibly zero-- doses for all available drugs) and then advances the simulation of time $t$.
Command $\Fun{get}(x)$ (with $x$ denoting one of the model variables) returns the value of model variable $x$ in the current state.

Since the input of our algorithm is a \digitaltwin \DT{\CR{C}} computed from a patient clinical record \CR{C} and consisting of a set of $n_p \in \IntegersGZ$ \Acp{VP} (see \cref{sec:digital-twin}), during the search we drive the simulation of $n_p$ \emph{independent copies} of our \Ac{VPH} model (each one connected to a copy of the monitor checking for treatment invariants and goals, as explained in \cref{sec:computing:monitor}). The different model copies are instantiated with different values for the model parameter vector defined in \DT{\CR{C}}, hence represent the different \Acp{VP} in the patient \digitaltwin. 

By means of commands $\Fun{run}(a,t)$ ($a \in A_1 \times \cdots \times A_{n_u}$), we simultaneously apply the same clinical action to \emph{all} \Acp{VP} in \DT{\CR{C}} and synchronously advance all models by time $t$. 
Furthermore, by means of $\Fun{store}$ and $\Fun{load}$ commands, we can efficiently expand a tree of sequences of clinical actions, as typically done by backtracking-based state exploration algorithms. In particular, upon a backtrack, we only need to load back a previously stored state of our models, thus avoiding to simulate the entire input sequence starting from the initial state.


==> 07.experimental-results/content.tex <==
%!TEX root = ../root.tex
%
In this section we outline how we set up and conducted our \Ac{ISCT} in order to assess the technical viability of the proposed approach.

\subsection{Retrospective clinical records}
\label{sec:isct:data}
\Input{data.tex}

\subsection{Computing \digitaltwins: exclusion criteria and \Acs{VP} selection}
\label{sec:isct:vp}
\Input{vp.tex}

\subsection{Multi-arm \Acl{ISCT} run}
\label{sec:isct:run}
\Input[run]{content.tex}




==> 07.experimental-results/data.tex <==
%!TEX root = ../root.tex
\begin{figure}
	\centering
	%
	\hfill
	\begin{subfigure}{\DataGet{paper/figures/subfigures/cols/2/width}}
		\IncludeGraphics
			[width=\linewidth]
			{figures/data/E2.pdf}
			%
			\caption{\Acs{E2}}
	\end{subfigure}
	\hfill
	\begin{subfigure}{\DataGet{paper/figures/subfigures/cols/2/width}}
		\IncludeGraphics
			[width=\linewidth]
			{figures/data/P4.pdf}
			%
			\caption{\Acs{P4}}
	\end{subfigure}
	\hfill
	
	\hfill
	\begin{subfigure}{\DataGet{paper/figures/subfigures/cols/2/width}}
		\IncludeGraphics
			[width=\linewidth]
			{figures/data/FSH.pdf}
			%
			\caption{\Acs{FSH}}
	\end{subfigure}
	\hfill
	\begin{subfigure}{\DataGet{paper/figures/subfigures/cols/2/width}}
		\IncludeGraphics
			[width=\linewidth]
			{figures/data/LH.pdf}
			%
			\caption{\Acs{LH}}
	\end{subfigure}
	\hfill

	
	\caption{Measurements (dots) of, respectively, \Ac{E2}, \Ac{P4}, \Ac{FSH} and \Ac{LH} of the 
		\DataGet{exps/results/clinicalrecords/all} 
	clinical records within the dataset from 
		\DataGet{exps/results/clinicalrecords/datasets}.
	}
	\label{fig:data}
\end{figure}


Our \Ac{ISCT} has been conducted against retrospective clinical data courtesy of \DataGet{exps/results/clinicalrecords/datasets}.

In particular, such our overall dataset consists of 
	\DataGet{exps/results/clinicalrecords/all} 
patient clinical records for a total of around 
	\DataGet{exps/results/clinicalrecords/measurements/all}
measurements.
%
Each clinical record comprises measurements for the hormones that play the most important role during the human menstrual cycle: \Ac{LH}, \Ac{FSH}, \Ac{E2}, and \Ac{P4}.
\Cref{fig:data} shows measurements of such hormones in our overall dataset.

Each of the 
	\DataGet{exps/results/clinicalrecords/all} 
clinical records in our retrospective clinical data defines a \emph{distinct arm} of our multi-arm \Ac{ISCT}.


==> 07.experimental-results/run/clinical-results.tex <==
%!TEX root = ../../root.tex

\begin{figure}
  \centering
  \IncludeGraphics[width=0.75\linewidth]{../figures/overall-drug-amount.pdf}
  \caption{Multi-arm \Ac{ISCT} outcomes.}
  \label{fig:isct:drug}
\end{figure}

\Cref{fig:isct:drug} shows the distribution of the total amount of drug employed by the optimal personalised treatments computed by our algorithm.
%
Note that, although we ran our multi-arm \Ac{ISCT} with a limited time budget and did not find provably \emph{lightest} treatments, the treatments we actually computed use, on average, less than \emph{half}
  (\DataGet{exps/results/average dose}) 
of the drug quantity employed by the reference treatment of \cref{sec:treatment} (\ie \Pretty{0.1}~mg on each day for up to \Pretty{30} days, totalling up to \Pretty{3}~mg and never less than \Pretty{2.8}~mg, since the required thresholds are never reached before day \Pretty{7}). 
%
As \cref{fig:isct:drug} shows, the computed treatments save, on average, 
  \DataGet{exps/results/average dose saving}
of the drug administered in the reference treatment (standard deviation: 
  \DataGet{exps/results/stddev}).

In \cref{fig:results}, we show our computed treatments for the 
  \DataGet{exps/results/clinicalrecords/all} 
patient clinical records during our multi-arm \Ac{ISCT}. 
%
We note that, the majority of the computed drug administration sequences is close to the reference downregulation treatment
in terms of administration frequency and treatment duration, \ie around \Pretty{28} days.
%
Besides this, there are also few computed treatments having a very light overall amount of drug dose. This of course depends on the ability of the \digitaltwins to capture patient peculiarities and in general on the ability of the \Ac{VPH} model at hand to represent the human physiology of interest.


\begin{figure}
  \centering
  \IncludeGraphics[width=\linewidth]{../figures/treatments.pdf}
  
  \caption{Personalised treatments computed through our multi-arm \Ac{ISCT} in 
    \DataGet{exps/results/computation/time/avg/days}.
  }

  \label{fig:results}
\end{figure}



==> 07.experimental-results/run/computational-results.tex <==
%!TEX root = ../../root.tex
We ran our multi-arm \Ac{ISCT} on the Marconi \Ac{HPC} infrastructure kindly provided by Cineca, Italy.
%
Due to CPU-hours budget limit, we ran each arm of our \Ac{ISCT} in parallel for 
	\DataGet{exps/results/computation/time/avg/days}. 
%
Each arm searches the optimal treatment for one of the 
	\DataGet{exps/results/clinicalrecords/all} 
patients in our dataset.
%
Indeed, our algorithm can be regarded as an \emph{any-time} algorithm in that, at any moment during search, it keeps track of the lightest successful treatment found so far.

\Cref{fig:computation:simulation-share} gives, for each \Ac{ISCT} arm, the share of simulation time within the whole computation time. 
%
As we already argued in \cref{sec:isct:vp}, the size of the input \digitaltwin highly impacts the speed (in terms of expanded search tree nodes per seconds) of our algorithm. 
In fact, in each search node (in the worst case), our algorithm needs to numerically simulate all \Acp{VP} within the input \digitaltwin.
As shown in \cref{fig:computation:simulation-share}, the time spent in carrying out simulations is, on average, the 
	\DataGet{exps/results/computation/simtime/avg/perc} 
of the total computation time.

This implies that any technique aimed at reducing the average number of simulations per search node (like the reduction of the size of the considered \digitaltwin defined in \cref{sec:isct:vp}, the action order heuristic evaluated in \cref{sec:isct:eval-action}, and the dynamic \Ac{VP} simulation ordering evaluated in \cref{sec:isct:eval-vp}) is expected to have a \emph{substantial impact} on the actual performance of the algorithm.



\begin{figure}
	\centering
	\hfill
    \begin{subfigure}{\DataGet{paper/figures/subfigures/cols/2/width}}
	    \IncludeGraphics[width=\linewidth]{../figures/times.pdf}

	    \caption{Time share of \digitaltwin simulations (dark bars) wrt. total computation time (dark  and light bars)}
	    \label{fig:computation:simulation-share}
	\end{subfigure}
	\hfill
    \begin{subfigure}{\DataGet{paper/figures/subfigures/cols/2/width}}
		\IncludeGraphics[width=\linewidth]{../figures/dt-nodes.pdf}
		\caption{Expanded search tree nodes (orange bars, left Y axis) vs.\ \digitaltwin sizes (blue bars, right Y axis)}
	    \label{fig:computation:dt-nodes}    
	\end{subfigure}
	
	\caption{Computational results of our \Ac{ISCT}.}
	\label{fig:computation}
\end{figure}



\Cref{fig:computation:dt-nodes} shows, for each of the 
	\DataGet{exps/results/clinicalrecords/all} 
parallel search processes (one per clinical record), the number of search nodes expanded within our time limit of 
	\DataGet{exps/results/computation/time/avg/days} 
(orange bars, left Y axis), and compares it to the size of the \digitaltwin considered for that clinical record (blue bars, right Y axis).

The figure show a \emph{clear negative correlation} (correlation coefficient equal to 
	\DataGet{exps/results/computation/correlation/dt nodes})
between number of expanded nodes within our time limit and the \digitaltwin size for all clinical records.
%
For example,
we note that when the \digitaltwin size is small, as for, \eg $\CR{C}_4$, the number of expanded nodes is large, \ie near \Pretty{e6}. Instead, when the \digitaltwin size is large, as for, \eg $\CR{C}_{17}$, the number of expanded nodes is quite low, \ie less than \Pretty{3e4}.



==> 07.experimental-results/run/content.tex <==
%!TEX root = ../../root.tex

We ran our 
	\DataGet{exps/results/clinicalrecords/all}-arm 
\Ac{ISCT} using a large \Ac{HPC} infrastructure (the Marconi cluster) kindly provided by the Cineca consortium. 

For each patient clinical record \CR{C} in our retrospective clinical data (see \cref{sec:data}), we, first, computed a \compactDT $\DTClusters{\CR{C}}$ (see \cref{sec:isct:vp}), and then we ran our algorithm of \cref{sec:computing} on an independent node of the cluster searching for an optimal (\ie lightest) and robust (\wrt \emph{all} \Acp{VP} of $\DTClusters{\CR{C}}$) downregulation treatment for \emph{that} specific \digitaltwin.
%
Thus, the whole 
	\DataGet{exps/results/clinicalrecords/all}-arm 
\Ac{ISCT} has been conducted in an \emph{embarrassing parallel fashion}.

Each \Ac{VP} in a \compactDT has been encoded in a Modelica (\url{http://www.modelica.org}) model (encompassing the GynCycle \Ac{VPH} model taking clinical actions as input, a parameter vector assignment, and a monitor to check for treatment invariants and goals) and has been simulated using JModelica v2.1 (\url{http://www.jmodelica.org}).
%
Our search algorithm (which drives a Modelica simulator per \Ac{VP}) has been implemented in Python.

In the following sections, we first evaluate the marginal impact of our heuristic ordering of actions (\cref{sec:isct:eval-action}) and of our dynamic simulation ordering of \Acp{VP} within a \digitaltwin (\cref{sec:isct:eval-vp}). 
Then, we present computational results (\cref{sec:isct:results:computation}) and outcomes (\cref{sec:isct:results:clinical}) of our multi-arm \Ac{ISCT}.


\subsubsection{Evaluation of the action ordering heuristic}
\label{sec:isct:eval-action}
\Input{eval-action.tex}


\subsubsection{Evaluation of the dynamic ordering of \Acsp{VP} within a \digitaltwin}
\label{sec:isct:eval-vp}
\Input{eval-vp.tex}


\subsubsection{Computational results}
\label{sec:isct:results:computation}
\Input{computational-results.tex}

\subsubsection{\Ac{ISCT} outcomes}
\label{sec:isct:results:clinical}
\Input{clinical-results.tex}


==> 07.experimental-results/run/eval-action.tex <==
%!TEX root = ../../root.tex
The goal of this section is to assess the marginal impact of the heuristic presented in \cref{sec:action:order}, which sorts actions by their ascending associated cost (administered drug dose), in the overall efficiency of the optimal personalised treatment search algorithm.

To this end, we compare it against
%the average behaviour of
\Pretty{10} runs of an action selection strategy that evaluates the possible actions in \emph{random} order when expanding each node of the search tree, and compare the performance of our heuristics against such reference strategy.

In particular, we defined a limit of \Pretty{e4} on the number of search tree nodes to expand, and
analysed how fast the cost (overall amount of drug dose) associated to the personalised treatments found \emph{decreases} during the search space exploration, on all \digitaltwins involved in our multi-arm \Ac{ISCT}.

In \cref{fig:eval-action}, we present \Pretty{3} representative executions where our heuristic finds an optimal solution at different points in time (\wrt the number of expanded search tree nodes). For convenience of presentation, the initial value of $D_{min}$ in \cref{fig:eval-action} is set to \Pretty{3.0} (drug quantity employed by the reference treatment, \ie \Pretty{0.1}~mg on each day for up to \Pretty{30} days) instead of $+\infty$ (as stated in \cref{sec:optimality}). This is in agreement with our exclusion criteria of \cref{sec:isct:vp} as the reference treatment succeed on all \Acp{VP} within our \digitaltwins.

We note that, by choosing actions randomly, the algorithm might show its first solution improvements a bit earlier (\cref{fig:eval-action-81,fig:eval-action-420}). However, in all cases, our heuristics finds the optimal solution (\ie the lightest treatment) within a number of expanded nodes which is \emph{orders of magnitude} lower than the number of expanded nodes required by the random action ordering strategy. As an example, \cref{fig:eval-action-420} shows that, after \Pretty{e4} expanded nodes, \Pretty{8} out of \Pretty{10} runs with the random action ordering still failed to find a solution better than the reference treatment (\ie \Pretty{3.0}~mg).


\begin{figure}
	\centering
	\hfill
	\begin{subfigure}{\DataGet{paper/figures/subfigures/cols/3/width}}
		\IncludeGraphics[width=\linewidth]
		{../figures/action-order/compare-81.pdf}
        \caption{}
        \label{fig:eval-action-81}
	\end{subfigure}
	\hfill
	\begin{subfigure}{\DataGet{paper/figures/subfigures/cols/3/width}}
		\IncludeGraphics[width=\linewidth]
		{../figures/action-order/compare-270.pdf}
        \caption{}
        \label{fig:eval-action-270}
	\end{subfigure}
	\hfill
	\begin{subfigure}{\DataGet{paper/figures/subfigures/cols/3/width}}
		\IncludeGraphics[width=\linewidth]
		{../figures/action-order/compare-420.pdf}
        \caption{}
        \label{fig:eval-action-420}
	\end{subfigure}
	\hfill

	\caption{Comparison of solution paths traversed by our algorithm when using our ordering heuristic (green line) against the references (red dashed lines) among different \digitaltwins of our multi-arm \Ac{ISCT}.}
	\label{fig:eval-action}
\end{figure}


==> 07.experimental-results/run/eval-vp.tex <==
%!TEX root = ../../root.tex
In order to evaluate the marginal impact of our dynamic \Ac{VP} simulation order within the input \digitaltwin (\cref{sec:order:vp}) at each search tree node, we compared the execution of our algorithm against a reference obtained by averaging \Pretty{10} different runs where the initial order of the \Acp{VP} is randomised and fixed at the beginning of the search.

In particular, we ran our algorithm for each \digitaltwin involved in our multi-arm \Ac{ISCT}, and compared the saving in terms of the number of simulations performed within each given number of search tree nodes.

\Cref{fig:eval-vp} shows our result on \Pretty{3} \digitaltwins having different sizes: 
(i)~a small size --- \Pretty{3} \Acp{VP} (\cref{fig:eval-vp-p3});
(ii)~an average size --- \Pretty{13} \Acp{VP} (\cref{fig:eval-vp-270});
and (iii)~a large size  --- \Pretty{36} \Acp{VP}(\cref{fig:eval-vp-541});
%
which are representative of the spectrum of behaviours among our \digitaltwins.

We note that the our dynamic \Ac{VP} simulation order is always beneficial. The highest saving in the number of simulations always occurs at the early stages of the search, where the most pruning activity is performed. In deeper stages of the search, the savings stabilise at values of the order of \Pretty{10}\%--\Pretty{20}\%.
Since the time needed to simulate a \Ac{VP} is essentially constant (as \Acp{VP} differ only in model parameter values and not in the system of \Aclp{ODE}, \Acsp{ODE}), such savings 
translate in comparable reductions of the overall computation time.
\AcronymReset{ODE}%

\begin{figure}
	\centering
    %
    \hfill
    \begin{subfigure}{\DataGet{paper/figures/subfigures/cols/3/width}}
        \IncludeGraphics[width=\linewidth]{../figures/vp-order/saving/compare-p3.pdf}
        \caption{}
        \label{fig:eval-vp-p3}
    \end{subfigure}
    \hfill
    \begin{subfigure}{\DataGet{paper/figures/subfigures/cols/3/width}}
        \IncludeGraphics[width=\linewidth]{../figures/vp-order/saving/compare-270.pdf}
        \caption{}
        \label{fig:eval-vp-270}
    \end{subfigure}
    \hfill
    \begin{subfigure}{\DataGet{paper/figures/subfigures/cols/3/width}}
        \IncludeGraphics[width=\linewidth]{../figures/vp-order/saving/compare-541.pdf}
        \caption{}
        \label{fig:eval-vp-541}
    \end{subfigure}
    \hfill
    
    \caption{Marginal impact of our dynamic \Ac{VP} simulation ordering strategy among the \digitaltwins of our multi-arm \Ac{ISCT}.}
    \label{fig:eval-vp}
\end{figure}


==> 07.experimental-results/vp.tex <==
%!TEX root = ../root.tex
%
From the GynCycle model, we generated a population $\Pop$ of around 
	\DataGet{exps/results/population}
\Acp{VP} as explained in \cite{mancini-etal:2014:fmcad,mancini-etal:2015:iwbbio} and recapped in \cref{sec:preliminaries:vp}. 
Hence, such a population is representative of (almost) all patient behaviours allowed by the model (in the sense of \cite{mancini-etal:2014:fmcad,mancini-etal:2015:iwbbio}).
%
Note that, although generating such a population required weeks of \Ac{HPC} computation, this is a one-time task for each \Ac{VPH} model.


In order to carry out our multi-arm \Ac{ISCT}, we computed a digital twin for each of the 
	\DataGet{exps/results/clinicalrecords/all} 
clinical records in our retrospective clinical data.
%
In particular, we set the threshold value $\delta$ (\cref{def:digitaltwin}) to 
	\DataGet{exps/results/mape} 
and, for each clinical record \CR{C}, we included in the \digitaltwin of \CR{C}, \DT{\CR{C}}, all $\lambda \in \Pop$ such that $\MAPE{\CR{C}}{\lambda} \leq 
	\DataGet{exps/results/mape}$.
%
Hence, for each clinical record, we selected \emph{all}
 \Acp{VP} having an average \Ac{MAPE} at most 
 	\DataGet{exps/results/mape}.

Since the reference downregulation treatment of \cref{sec:treatment} does not succeed on all possible phenotypes (this is not surprising since, as described in \cref{sec:treatment}, fertility treatments are known to have a low rate of success), we removed from \DT{\CR{C}} those \Acp{VP} for which the treatment using the maximum allowed dose (\ie \Pretty{0.1}~mg on each day for up to \Pretty{30} days, see \cref{sec:treatment}) fails, for any \CR{C}.
%
Such an \emph{exclusion criterion} directly stems from domain knowledge on downregulation treatments (namely: for these protocols, if a treatment envisioning one full drug dose per day fails for a patient, a lighter treatment will fail as well).
%
Our 
	\DataGet{exps/results/clinicalrecords/all} 
digital twins contain, on average, 
	\DataGet{exps/results/computation/dt/size/avg} 
\Acp{VP} each.

Unfortunately, in the worst-case scenario, each step of our backtracking search requires to simulate all \Acp{VP} within the input \digitaltwin in order to check the monitor output (\ie treatment invariants and goals, see \cref{sec:safety}).
%
Thus, since simulating one \Ac{VP} requires seconds of numerical integration, the total computation time of our algorithm is highly affected by the size of the input \digitaltwin, and may easily become impractical.

To overcome such an obstacle, we note that within a \digitaltwin of a given clinical record we can (and typically do) have \Acp{VP} exhibiting very similar model behaviours (both with and without drug administrations). Simulating such very similar \Acp{VP} would then simply be a waste of computation as long as our \Ac{ISCT} is concerned.
%
In order to reduce the size of a \digitaltwin, we compute a subset $\DTClusters{\CR{C}}$ of \DT{\CR{C}}, for each given clinical record \CR{C}, such that $\DTClusters{\CR{C}}$ does not contain such \emph{redundant} \Acp{VP}.

To do so, we define the \emph{distance} among the time evolutions of any biological quantity $S_i$ ($i \in [n_x]$) of two \Acp{VP} normalised against the time evolution of $S_i$ of a third (reference) \Ac{VP} (\cref{def:distance}).

\begin{definition}
\label{def:distance}
Let $\lambda, \lambda'$ and $\lambda^\star$ be three \Acp{VP} of a \Ac{VPH} model defining $n_x$ biological quantities.

For every biological quantity $S_i$ ($i \in [n_x]$)
the \emph{distance} between $\lambda$ and $\lambda'$ \wrt $\lambda^\star$ on $S_i$ is:

\begin{align*}
d_{i, \lambda^\star}(\lambda, \lambda') =
\frac{
	\sqrt{
		\int_{0}^{+\infty} {
			\left[ x_i(\lambda, t) - x_i(\lambda', t) \right]^2 
				~\text{d}t
		}
	}
}{ \zeta\left( \sqrt{
		\int_{0}^{+\infty} {
			x_i(\lambda^\star, t)^2 ~\text{d}t
		}
	}\right)
}
\end{align*}
%
where, as usual, $\zeta(\alpha)$ is $\alpha$ when $\alpha \neq \Pretty{0}$ and a small constant otherwise (in order to avoid division by \Pretty{0}).
\end{definition}

Intuitively, \cref{def:distance} defines the \emph{Euclidean distance} between the time evolutions of biological quantity $S_i$ of two given \Acp{VP} ($\lambda$ and $\lambda'$) \emph{normalised} \wrt the $L_2$-norm of that of a \emph{reference} \Ac{VP}, $\lambda^\star$.
%
In practice, we will compute the above distance using a bounded-horizon simulation, \ie model trajectories will be defined for $0 \leq t \leq h$, where $h$ is the treatment horizon. Hence, to match the above general definition, we assume that, for any $t > h$, $x_i(\lambda^\star,t)$, $x_i(\lambda,t)$ and $x_i(\lambda',t)$ are \Pretty{0}.


Given this notion of distance, 
we build $\DTClusters{\CR{C}}$ from the \digitaltwin \DT{\CR{C}} of a clinical record \CR{C} as follows:
\begin{itemize}
\item We select, from \DT{\CR{C}}, the reference \Ac{VP} $\lambda^\star$ as one that \emph{minimises} $\MAPE{\CR{C}}{\lambda^\star}$. In other words, $\lambda^\star$ is one of the \Acp{VP} of $\Pop$ that \emph{best matches} the clinical measurements of \CR{C}.

\item We \emph{remove} from \DT{\CR{C}} those \Acp{VP} whose time evolutions of \emph{all} biological quantities have a distance below a certain threshold from other \Acp{VP} in $\DTClusters{\CR{C}}$ \wrt $\lambda^\star$ (\cref{def:selection}). 
\end{itemize}
%
Such a distance threshold obviously depends on the \Ac{VPH} model and treatment subject of the \Ac{ISCT}.

\begin{definition}
\label{def:selection}
Let \CR{C} be a patient clinical record,
\DT{\CR{C}} be its \digitaltwin,
$\lambda^\star$ be any \Ac{VP} such that $\MAPE{\CR{C}}{\lambda^\star}$ is minimal,
and
$d$ be the distance function of \cref{def:distance}.

Then, given a threshold $\theta$, we call \emph{\compactDT} $\DTClusters{\CR{C}}$ \emph{any} subset of $\DT{\CR{C}}$ such that the following condition holds: 

\begin{align*}
\forall \lambda \in \DT{\CR{C}} \: . \: 
	\lambda \not\in \DTClusters{\CR{C}} \rightarrow 
		\exists \lambda' \in \DTClusters{\CR{C}} \: . \: 
			\forall i \in [n_x] \: 
				d_{i, \lambda^\star}(\lambda, \lambda') 
				\leq \theta/2.
\end{align*}
\end{definition}

As a result of the application of the above approach and of our exclusion criteria, we obtained \compactDTs with an average size of 
	\DataGet{exps/results/computation/dt/clusters/num/avg}. 
%
This has been achieved by tuning the distance threshold $\theta$ in such a way that:
(i)~\Acp{VP} having redundant and undistinguishable behaviours have been filtered out;
(ii)~the computed \compactDTs were representative enough for all \Acp{VP} in corresponding patient \digitaltwins;
and (iii)~their sizes were small enough to be computationally affordable.
%
\Cref{fig:digitaltwin-distr} shows the distribution of their sizes.



\begin{figure}
	\centering
	\IncludeGraphics[width=0.7\linewidth]{figures/data/dt.pdf}
	\caption{
	  Bar chart showing \digitaltwin sizes (in terms of number of \Acp{VP}) before (light) and after (dark) the removal of redundant \Acp{VP} and the application of our exclusion criteria for each clinical record.
	}
	\label{fig:digitaltwin-distr}
\end{figure}



==> 08.conclusions/content.tex <==
%!TEX root = ../root.tex
In this paper we presented methods and algorithms based on intelligent search aimed at synthesising optimal personalised treatments by means of \Acp{ISCT}, exploiting quantitative models of the physiology and drugs \Ac{PKPD} of interest, and clinical measurements on human patients from which we define their \digitaltwins.

We applied our approach on a case study involving a complex state-of-the-art model of the human female \Ac{HPG} axis, in order to compute, for any given patient, a \emph{personalised treatment} for the downregulation phase of an assisted reproduction protocol, which is effective on the patient at hand, but minimises the overall amount of drug used (hence, indirectly, the associated cost as well as likelihood and severity of adverse effects). 

The possibility to \emph{optimise} \insilico, in a few weeks of computation on a \Ac{HPC} infrastructure, a complex treatment for a \emph{given} human patient \emph{before} its actual administration shows the potential of artificial intelligence for model-based (\insilico) precision medicine.
This however calls for \emph{trusted} \Ac{VPH} models, which is currently one of the major obstacles for the uptake of \Acp{ISCT} in clinical practice.

Indeed, the results of our \Ac{ISCT} (conducted using a state-of-the-art \emph{validated} \Ac{VPH} model as GynCycle) are extremely promising, but must be taken with care.  
In particular, an \invivo evaluation of the actual effectiveness of the personalised treatments generated by our algorithm is needed in order to assess the accuracy of GynCycle in predicting the patient reactions to \emph{non-standard drug dosing patterns}, as those computed by our algorithm. 




==> abstract.tex <==
%!TEX root = ./root.tex

\Acp{ISCT}, \ie clinical experimental campaigns carried out by means of computer simulations, hold the promise to decrease time and cost for the safety and efficacy assessment of pharmacological treatments, reduce the need for animal and human testing, and enable precision medicine.%, where personalised treatments optimised for each patient can be designed before being actually administered.

In this paper we present methods and an algorithm that, by means of extensive computer simulation--based experimental campaigns (\Acp{ISCT}) guided by intelligent search, optimise a pharmacological treatment for an individual patient (\emph{precision medicine}).
%
We show the effectiveness of our approach on a case study involving a real pharmacological treatment, namely the \emph{downregulation} phase of a complex clinical protocol for assisted reproduction in humans.

==> bibliography.tex <==
\providecommand{\MCLabProceedingsOf}[1]{Proceedings of #1}
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi:\discretionary{}{}{}#1}\else
  \providecommand{\doi}{doi:\discretionary{}{}{}\begingroup
  \urlstyle{rm}\Url}\fi
\providecommand{\eprint}[2][]{\url{#2}}

\bibitem{mancini-etal:2018:rcra-treatment}
Mancini T, Mari F, Massini A, Melatti I, Salvo I, Sinisi S, Tronci E, Ehrig R,
  R{\"{o}}blitz S, Leeners B.
\newblock Computing Personalised Treatments through In Silico Clinical Trials.
  {{A}} Case Study on Downregulation in Assisted Reproduction.
\newblock In: \MCLabProceedingsOf{25th RCRA International Workshop on
  Experimental Evaluation of Algorithms for Solving Problems with Combinatorial
  Explosion (RCRA~2018)}, volume 2271 of \emph{CEUR Workshop Proceedings}.
  CEUR-WS.org, 2018.

\bibitem{mould-etal:2012:pkpd}
Mould D, Upton R.
\newblock Basic Concepts in Population Modeling, Simulation, and Model-Based
  Drug Development.
\newblock \emph{CPT: Pharmacometrics \& Systems Pharmacology}, 2012.
\newblock \textbf{1}(9):1--14.

\bibitem{clapworthy-etal:2007:vph}
Clapworthy G, Kohl P, Gregerson H, Thomas S, Viceconti M, Hose D, Pinney D,
  Fenner J, McCormack K, Lawford P, Van Sint~Jan S, Waters S, Coveney P.
\newblock Digital Human Modelling: A Global Vision and a European Perspective.
\newblock In: Duffy V (ed.), Digital Human Modeling. Springer, Berlin,
  Heidelberg.
\newblock ISBN 978-3-540-73321-8, 2007 pp. 549--558.

\bibitem{trayanova-etal:2018:curr-opin-biomed-eng}
Trayanova N, Boyle P, Nikolov P.
\newblock Personalized imaging and modeling strategies for arrhythmia
  prevention and therapy.
\newblock \emph{Current Opinion in Biomedical Engineering}, 2018.
\newblock \textbf{5}:21--28.
\newblock \doi{10.1016/j.cobme.2017.11.007}.

\bibitem{cox-etal:2009:circulatory}
Cox L, Loerakker S, Rutten M, De~Mol B, Van De~Vosse F.
\newblock A Mathematical Model to Evaluate Control Strategies for Mechanical
  Circulatory Support.
\newblock \emph{Artificial Organs}, 2009.
\newblock \textbf{33}(8):593--603.
\newblock \doi{10.1111/j.1525-1594.2009.00755.x}.

\bibitem{roeblitz-etal:2013:theorbio}
R\"{o}blitz S, St\"{o}tzel C, Deuflhard P, Jones H, Azulay DO, van~der Graaf P,
  Martin S.
\newblock A Mathematical Model of the Human Menstrual Cycle for the
  Administration of {GnRH} Analogues.
\newblock \emph{Journal of Theoretical Biology}, 2013.
\newblock \textbf{321}:8--27.
\newblock \doi{http://dx.doi.org/10.1016/j.jtbi.2012.11.020}.

\bibitem{ribba-etal:2012:tumor}
Ribba B, Kaloshi G, Peyre M, Ricard D, Calvez V, Tod M, {\v{C}}ajavec-Bernard
  B, Idbaih A, Psimaras D, Dainese L, Pallud J, Cartalat-Carel S, Delattre JY,
  Honnorat J, Grenier E, Ducray F.
\newblock A Tumor Growth Inhibition Model for Low-Grade Glioma Treated with
  Chemotherapy or Radiotherapy.
\newblock \emph{Clinical Cancer Research}, 2012.
\newblock \textbf{18}(18):5071--5080.
\newblock \doi{10.1158/1078-0432.CCR-12-0084}.

\bibitem{jackson-etal:2015:neuro}
Jackson P, Juliano J, Hawkins-Daarud A, Rockne R, Swanson K.
\newblock Patient-Specific Mathematical Neuro-Oncology: Using a Simple
  Proliferation and Invasion Tumor Model to Inform Clinical Practice.
\newblock \emph{Bulletin of Mathematical Biology}, 2015.
\newblock \textbf{77}(5):846--856.
\newblock \doi{10.1007/s11538-015-0067-7}.

\bibitem{roy-etal:2010:jpp}
Roy P, Roy K.
\newblock Molecular docking and {QSAR} studies of aromatase inhibitor
  androstenedione derivatives.
\newblock \emph{Journal of Pharmacy and Pharmacology}, 2010.
\newblock \textbf{62}(12):1717--1728.
\newblock \doi{10.1111/j.2042-7158.2010.01154.x}.

\bibitem{bachler-etal:2014:species}
B{\"{a}}chler M, Menshykau D, De~Geyter C, Iber D.
\newblock Species-Specific Differences in Follicular Antral Sizes Result from
  Diffusion-Based Limitations on the Thickness of the Granulosa Cell Layer.
\newblock \emph{Molecular Human Reproduction}, 2014.
\newblock \textbf{20}(3):208--221.
\newblock \doi{10.1093/molehr/gat078}.

\bibitem{iarosz-etal:2015:jtb}
Iarosz K, Borges F, Batista A, Baptista M, Siqueira R, Viana R, Lopes S.
\newblock Mathematical model of brain tumour with glia--neuron interactions and
  chemotherapy treatment.
\newblock \emph{Journal of Theoretical Biology}, 2015.
\newblock \textbf{368}:113--121.
\newblock \doi{10.1016/j.jtbi.2015.01.006}.

\bibitem{yalcinkaya:2013:eleco}
Yalcinkaya F, Kizilkaplan E, Erbas A.
\newblock Mathematical modelling of human heart as a hydroelectromechanical
  system.
\newblock In: \MCLabProceedingsOf{8th International Conference on Electrical
  and Electronics Engineering (ELECO~2013)}. IEEE, 2013 pp. 362--366.
\newblock \doi{10.1109/ELECO.2013.6713862}.

\bibitem{muller:2014:ijnmbe}
M{\"{u}}ller LO, Toro EF.
\newblock A global multiscale mathematical model for the human circulation with
  emphasis on the venous system.
\newblock \emph{International Journal for Numerical Methods in Biomedical
  Engineering}, 2014.
\newblock \textbf{30}(7):681--725.
\newblock \doi{10.1002/cnm.2622}.

\bibitem{kanderian-etal:2009:jdst}
Kanderian S, Weinzimer S, Voskanyan G, Steil G.
\newblock Identification of Intraday Metabolic Profiles during Closed-Loop
  Glucose Control in Individuals with Type 1 Diabetes.
\newblock \emph{Journal of Diabetes Science and Technology}, 2009.
\newblock \textbf{3}:1047--1057.
\newblock \doi{10.1177/193229680900300508}.

\bibitem{herrero-etal:2013:jdst}
Herrero P, Georgiou P, Oliver N, Reddy M, Johnston D, Toumazou C.
\newblock A Composite Model of Glucagon--Glucose Dynamics for In Silico Testing
  of Bihormonal Glucose Controllers.
\newblock \emph{Journal of Diabetes Science and Technology}, 2013.
\newblock \textbf{7}:941--951.
\newblock \doi{10.1177/193229681300700416}.

\bibitem{dallaman-etal:2014:jdst}
Dalla~Man C, Micheletto F, Lv D, Breton M, Kovatchev B, Cobelli C.
\newblock The {{UVA}}/{{Padova}} Type 1 Diabetes Simulator: New Features.
\newblock \emph{Journal of Diabetes Science and Technology}, 2014.
\newblock \textbf{8}:26--34.
\newblock \doi{10.1177/1932296813514502}.

\bibitem{schaller-etal:2013:glucose}
Schaller S, Willmann S, Lippert J, Schaupp L, Pieber T, Schuppert A, Eissing T.
\newblock A generic integrated physiologically based whole-body model of the
  glucose-insulin-glucagon regulatory system.
\newblock \emph{{CPT}: Pharmacometrics \& Systems Pharmacology}, 2013.
\newblock \textbf{2}(8):1--10.
\newblock \doi{10.1038/psp.2013.40}.

\bibitem{schlender-etal:2016:clinpharm}
Schlender JF, Meyer M, Thelen K, Krauss M, Willmann S, Eissing T, Jaehde U.
\newblock Development of a Whole-Body Physiologically Based Pharmacokinetic
  Approach to Assess the Pharmacokinetics of Drugs in Elderly Individuals.
\newblock \emph{Clinical Pharmacokinetics}, 2016.
\newblock \textbf{55}(12):1573--1589.

\bibitem{hester-etal:2011:frontphysiol}
Hester R, Brown A, Husband L, Iliescu R, Pruett W, Summers R, Coleman T.
\newblock HumMod: a modeling environment for the simulation of integrative
  human physiology.
\newblock \emph{Frontiers in physiology}, 2011.
\newblock \textbf{2}:12.

\bibitem{matejak-etal:2015:embc}
Matej{\'{a}}k M, Kofr{\'{a}}nek J.
\newblock Physiomodel -- {A}n integrative physiology in {M}odelica.
\newblock In: \MCLabProceedingsOf{37th Annual International Conference of the
  IEEE Engineering in Medicine and Biology Society (EMBC~2015)}. IEEE, 2015 pp.
  1464--1467.

\bibitem{hucka-etal:2003:bioinf}
Hucka M, Finney A, Sauro HM, Bolouri H, Doyle JC, Kitano H, Arkin AP, Bornstein
  BJ, Bray D, Cornish-Bowden A, Cuellar AA, Dronov S, Gilles ED, Ginkel M, Gor
  V, Goryanin II, Hedley WJ, Hodgman TC, Hofmeyr JH, Hunter PJ, Juty NS,
  Kasberger JL, Kremling A, Kummer U, Le~Nov{\`{e}}re N, Loew LM, Lucio D,
  Mendes P, Minch E, Mjolsness ED, Nakayama Y, Nelson MR, Nielsen PF, Sakurada
  T, Schaff JC, Shapiro BE, Shimizu TS, Spence HD, Stelling J, Takahashi K,
  Tomita M, Wagner J, Wang J.
\newblock The {S}ystems {B}iology {M}arkup language ({SBML}): a medium for
  representation and exchange of biochemical network models.
\newblock \emph{Bioinformatics}, 2003.
\newblock \textbf{19}(4):524--531.
\newblock \doi{10.1093/bioinformatics/btg015}.

\bibitem{yoshiyuki-etal:2014:phml}
Asai Y, Abe T, Oka H, Okita M, Hagihara K, Ghosh S, Matsuoka Y, Kurachi Y,
  Nomura T, Kitano H.
\newblock A Versatile Platform for Multilevel Modeling of Physiological
  Systems: {SBML-PHML} Hybrid Modeling and Simulation.
\newblock \emph{Advances Biomedical Engineering}, 2014.
\newblock \textbf{3}:50--58.
\newblock \doi{10.14326/abe.3.50}.

\bibitem{fritzson-etal:2007:biochem}
Fritzson P, Ulfhielm E, Belic A, Fransson M, Gr{\`{e}}en H.
\newblock Biochemical Mathematical Modeling with Modelica and the BioChem
  Library.
\newblock In: \MCLabProceedingsOf{6th International Conference on Applied
  Mathematics (APLIMAT~2007)}. 2007 pp. 147--159.

\bibitem{maggioli-etal:2019:bioinf}
Maggioli F, Mancini T, Tronci E.
\newblock {SBML2Modelica}: Integrating Biochemical Models within Open-Standard
  Simulation Ecosystems.
\newblock \emph{Bioinformatics}, 2019.
\newblock \doi{10.1093/bioinformatics/btz860}.

\bibitem{avicenna:2016:roadmap}
{Avicenna Project}.
\newblock \emph{In silico} Clinical Trials: How Computer Simulation will
  Transform the Biomedical Industry.
\newblock
  \url{http://avicenna-isct.org/wp-content/uploads/2016/01/AvicennaRoadmapPDF-27-01-16.pdf},
  2016.

\bibitem{pappalardo-etal:2018:insilico}
Pappalardo F, Russo G, Tshinanu F, Viceconti M.
\newblock \emph{In silico} clinical trials: concepts and early adoptions.
\newblock \emph{Briefings in Bioinformatics}, 2018.
\newblock \doi{10.1093/bib/bby043}.

\bibitem{weld:1999:planning}
Weld D.
\newblock Recent Advances in AI Planning.
\newblock \emph{AI Magazine}, 1999.
\newblock \textbf{20}(2):93--93.

\bibitem{rossi-etal:2006:constraint}
Rossi F, Van~Beek P, Walsh T (eds.).
\newblock Handbook of Constraint Programming.
\newblock Elsevier, 2006.

\bibitem{biere-etal:2009:sat}
Biere A, Heule M, van Maaren H (eds.).
\newblock Handbook of Satisfiability, volume 185.
\newblock IOS Press, 2009.

\bibitem{sontag:1998:book}
Sontag E.
\newblock Mathematical Control Theory: Deterministic Finite Dimensional Systems
  (2nd Ed.).
\newblock Springer, 1998.
\newblock ISBN 0-387-984895.

\bibitem{alur-etal:2001:hscc}
Alur R, Belta C, Ivan{\v{c}}i{\'{c}} F, Kumar V, Mintz M, Pappas GJ, Rubin H,
  Schug J.
\newblock Hybrid Modeling and Simulation of Biomolecular Networks.
\newblock In: \MCLabProceedingsOf{4th International Workshop on Hybrid Systems:
  Computation and Control (HSCC~2001)}, volume 2034 of \emph{Lecture Notes in
  Computer Science}. Springer, 2003 pp. 19--32.
\newblock \doi{10.1007/3-540-45351-2_6}.

\bibitem{bartocci-etal:2016:plos-comp-bio}
Bartocci E, Li{\'{o}} P.
\newblock Computational modeling, formal analysis, and tools for systems
  biology.
\newblock \emph{PLoS Computational Biology}, 2016.
\newblock \textbf{12}(1):e1004591.
\newblock \doi{10.1371/journal.pcbi.1004591}.

\bibitem{wang-etal:2016:hldvt}
Wang Q, Clarke EM.
\newblock Formal modeling of biological systems.
\newblock In: \MCLabProceedingsOf{2016 IEEE International High Level Design
  Validation and Test Workshop (HLDVT)}. IEEE, 2016 pp. 178--184.
\newblock \doi{10.1109/HLDVT.2016.7748273}.

\bibitem{mancini-etal:2017:ipl}
Mancini T, Mari F, Massini A, Melatti I, Salvo I, Tronci E.
\newblock On Minimising the Maximum Expected Verification Time.
\newblock \emph{Information Processing Letters}, 2017.
\newblock \textbf{122}:8--16.
\newblock \doi{10.1016/j.ipl.2017.02.001}.

\bibitem{mancini-etal:2014:fmcad}
Tronci E, Mancini T, Salvo I, Sinisi S, Mari F, Melatti I, Massini A, Dav{i'}
  F, Dierkes T, Ehrig R, R{\"{o}}blitz S, Leeners B, Kr{\"{u}}ger T, Egli M,
  Ille F.
\newblock Patient-Specific Models from Inter-Patient Biological Models and
  Clinical Records.
\newblock In: \MCLabProceedingsOf{14th International Conference on Formal
  Methods in Computer-Aided Design (FMCAD 2014)}. IEEE, 2014 pp. 207--214.
\newblock \doi{10.1109/FMCAD.2014.6987615}.

\bibitem{mancini-etal:2015:iwbbio}
Mancini T, Tronci E, Salvo I, Mari F, Massini A, Melatti I.
\newblock Computing Biological Model Parameters by Parallel Statistical Model
  Checking.
\newblock In: \MCLabProceedingsOf{3rd International Conference on
  Bioinformatics and Biomedical Engineering (IWBBIO~2015)}, volume 9044 of
  \emph{Lecture Notes in Computer Science}. Springer, 2015 pp. 542--554.
\newblock \doi{10.1007/978-3-319-16480-9_52}.

\bibitem{calabrese-etal:2019:rcra}
Calabrese A, Mancini T, Massini A, Sinisi S, Tronci E.
\newblock Generating {T1DM} Virtual Patients for In Silico Clinical Trials via
  {AI}-Guided Statistical Model Checking.
\newblock In: \MCLabProceedingsOf{26th RCRA International Workshop on
  Experimental Evaluation of Algorithms for Solving Problems with Combinatorial
  Explosion (RCRA~2019)}, volume 2538 of \emph{CEUR Workshop Proceedings}.
  CEUR-WS.org, 2019 .

\bibitem{leeners-etal:2017:behavioral}
Leeners B, Kruger T, Geraedts K, Tronci E, Mancini T, Ille F, Egli M, Roeblitz
  S, Saleh L, Spanaus K, Schippert C, Zhang Y, Hengartner M.
\newblock Lack of Associations between Female Hormone Levels and Visuospatial
  Working Memory, Divided Attention and Cognitive Bias across Two Consecutive
  Menstrual Cycles.
\newblock \emph{Frontiers in Behavioral Neuroscience}, 2017.
\newblock \textbf{11}.
\newblock \doi{10.3389/fnbeh.2017.00120}.

\bibitem{hengartner-etal:2017:psycho}
Hengartner M, Kruger T, Geraedts K, Tronci E, Mancini T, Ille F, Egli M,
  Roeblitz S, Ehrig R, Saleh L, Spanaus K, Schippert C, Zhang Y, Leeners B.
\newblock Negative Affect is Unrelated to Fluctuations in Hormone Levels Across
  the Menstrual Cycle: Evidence from a Multisite Observational Study across Two
  Successive Cycles.
\newblock \emph{Journal of Psychosomatic Research}, 2017.
\newblock \textbf{99}:21--27.
\newblock \doi{10.1016/j.jpsychores.2017.05.018}.

\bibitem{leeners-etal:2019:front-psychol}
Leeners B, Kr{\"{u}}ger T, Geraedts K, Tronci E, Mancini T, Egli M,
  R{\"{o}}blitz S, Saleh L, Spanaus K, Schippert C, Zhang Y, Ille F.
\newblock Associations Between Natural Physiological and Supraphysiological
  Estradiol Levels and Stress Perception.
\newblock \emph{Frontiers in Psychology}, 2019.
\newblock \textbf{10}:1296.
\newblock \doi{10.3389/fpsyg.2019.01296}.

\bibitem{mancini-etal:2013:cav}
Mancini T, Mari F, Massini A, Melatti I, Merli F, Tronci E.
\newblock System Level Formal Verification via Model Checking Driven
  Simulation.
\newblock In: \MCLabProceedingsOf{25th International Conference on Computer
  Aided Verification (CAV~2013)}, volume 8044 of \emph{Lecture Notes in
  Computer Science}. Springer, 2013 pp. 296--312.
\newblock \doi{10.1007/978-3-642-39799-8_21}.

\bibitem{mancini-etal:2016:micpro}
Mancini T, Mari F, Massini A, Melatti I, Tronci E.
\newblock Anytime System Level Verification via Parallel Random Exhaustive
  Hardware in the Loop Simulation.
\newblock \emph{Microprocessors and Microsystems}, 2016.
\newblock \textbf{41}:12--28.
\newblock \doi{10.1016/j.micpro.2015.10.010}.

\bibitem{mancini-etal:2014:dsd-anytime}
Mancini T, Mari F, Massini A, Melatti I, Tronci E.
\newblock Anytime System Level Verification via Random Exhaustive Hardware In
  The Loop Simulation.
\newblock In: \MCLabProceedingsOf{17th Euromicro Conference on Digital System
  Design (DSD~2014)}. IEEE, 2014 pp. 236--245.

\bibitem{mancini-etal:2015:sylvaas-pdp}
Mancini T, Mari F, Massini A, Melatti I, Tronci E.
\newblock {SyLVaaS}: System Level Formal Verification as a Service.
\newblock In: \MCLabProceedingsOf{23rd Euromicro International Conference on
  Parallel, Distributed, and Network-Based Processing (PDP~2015)}. IEEE, 2015
  pp. 476--483.

\bibitem{mancini-etal:2014:pdp}
Mancini T, Mari F, Massini A, Melatti I, Tronci E.
\newblock System Level Formal Verification via Distributed Multi-Core Hardware
  in the Loop Simulation.
\newblock In: \MCLabProceedingsOf{22nd Euromicro International Conference on
  Parallel, Distributed, and Network-Based Processing (PDP~2014)}. IEEE, 2014
  pp. 734--742.
\newblock \doi{10.1109/PDP.2014.32}.

\bibitem{mancini-etal:2016:fundam}
Mancini T, Mari F, Massini A, Melatti I, Tronci E.
\newblock {SyLVaaS}: System Level Formal Verification as a Service.
\newblock \emph{Fundamenta Informaticae}, 2016.
\newblock \textbf{1--2}:101--132.
\newblock \doi{10.3233/FI-2016-1444}.

\bibitem{mancini-etal:2012:sac}
Mancini T, Flener P, Pearson J.
\newblock Combinatorial Problem Solving over Relational Databases: View
  Synthesis through Constraint-Based Local Search.
\newblock In: \MCLabProceedingsOf{{ACM} Symposium on Applied Computing
  (SAC~2012)}. ACM, 2012 pp. 80--87.
\newblock \doi{10.1145/2245276.2245295}.

\bibitem{glover-etal:2006:metaheuristics}
Glover F, Kochenberger G (eds.).
\newblock Handbook of Metaheuristics, volume~57.
\newblock Springer, 2006.

\bibitem{gottlob-etal:2007:conditional}
Gottlob G, Greco G, Mancini T.
\newblock Conditional Constraint Satisfaction: Logical Foundations and
  Complexity.
\newblock In: \MCLabProceedingsOf{20th International Joint Conference on
  Artificial Intelligence (IJCAI~2007)}. 2007 pp. 88--93.

\bibitem{mancini-etal:2008:constraints}
Mancini T, Cadoli M, Micaletto D, Patrizi F.
\newblock Evaluating {ASP} and Commercial Solvers on the {CSPLib}.
\newblock \emph{Constraints}, 2008.
\newblock \textbf{13}(4):407--436.

\bibitem{bordeaux-etal:2008:jair}
Bordeaux L, Cadoli M, Mancini T.
\newblock A Unifying Framework for Structural Properties of {CSP}s:
  Definitions, Complexity, Tractability.
\newblock \emph{Journal of Artificial Intelligence Research}, 2008.
\newblock \textbf{32}:607--629.
\newblock \doi{10.1613/jair.2538}.

\bibitem{bordeaux-etal:2009:tocl}
Bordeaux L, Cadoli M, Mancini T.
\newblock Generalizing Consistency and other Constraint Properties to
  Quantified Constraints.
\newblock \emph{{ACM} Transactions on Computational Logic}, 2009.
\newblock \textbf{10}(3):17:1--17:25.
\newblock \doi{10.1145/1507244.1507247}.

\bibitem{raghupathi-etal:2014:hiss}
Raghupathi W, Raghupathi V.
\newblock Big data analytics in healthcare: promise and potential.
\newblock \emph{Health Information Science and Systems}, 2014.
\newblock \textbf{2}(1):3.
\newblock \doi{10.1186/2047-2501-2-3}.

\bibitem{fogliata-etal:2014:radonc}
Fogliata A, Belosi F, Clivio A, Navarria P, Nicolini G, Scorsetti M, Vanetti E,
  Cozzi L.
\newblock On the pre-clinical validation of a commercial model-based
  optimisation engine: Application to volumetric modulated arc therapy for
  patients with lung or prostate cancer.
\newblock \emph{Radiotherapy \& Oncology}, 2014.
\newblock \textbf{113}(3):385--391.
\newblock \doi{10.1016/j.radonc.2014.11.009}.

\bibitem{willmann-etal:2003:biosilico}
Willmann S, Lippert J, Sevestre M, Solodenko J, Fois F, Schmitt W.
\newblock {PK-Sim}\textsuperscript{{$\textregistered$}}: a physiologically
  based pharmacokinetic 'whole-body' model.
\newblock \emph{{BIOSILICO}}, 2003.
\newblock \textbf{1}(4):121--124.
\newblock \doi{10.1016/S1478-5382(03)02342-4}.

\bibitem{jeena-etal:2011:aac}
Jeena P, Bishai W, Pasipanodya J, Gumbo T.
\newblock \emph{In Silico} children and the glass mouse model: clinical trial
  simulations to identify and individualize optimal isoniazid doses in children
  with tuberculosis.
\newblock \emph{Antimicrobial Agents and Chemotherapy}, 2011.
\newblock \textbf{55}(2):539--545.
\newblock \doi{10.1128/AAC.00763-10}.

\bibitem{dijkman-etal:2018:cpt}
van Dijkman S, Wicha S, Danhof M, Della~Pasqua O.
\newblock Individualized dosing algorithms and therapeutic monitoring for
  antiepileptic drugs.
\newblock \emph{Clinical Pharmacology \& Therapeutics}, 2018.
\newblock \textbf{103}(4):663--673.
\newblock \doi{10.1002/cpt.777}.

\bibitem{lenovere:2015:nrg}
Le~Nov{\`{e}}re N.
\newblock Quantitative and logic modelling of molecular and gene networks.
\newblock \emph{Nature Reviews Genetics}, 2015.
\newblock \textbf{16}(3):146--158.
\newblock \doi{10.1038/nrg3885}.

\bibitem{fox-etal:2006:jair}
Fox M, Long D.
\newblock Modelling Mixed Discrete-Continuous Domains for Planning.
\newblock \emph{Journal of Artificial Intelligence Research}, 2006.
\newblock \textbf{27}:235--297.

\bibitem{vallati-etal:2016:aaai}
Vallati M, Magazzeni D, De~Schutter B, Chrpa L, McCluskey T.
\newblock Efficient Macroscopic Urban Traffic Models for Reducing Congestion: A
  {PDDL+} Planning Approach.
\newblock In: \MCLabProceedingsOf{30th National Conference on Artificial
  Intelligence (AAAI~2016)}. AAAI, 2016 pp. 3188--3194.

\bibitem{coles-etal:2014:icaps}
Coles A, Coles A.
\newblock {PDDL+} Planning with Events and Linear Processes.
\newblock In: \MCLabProceedingsOf{24th International Conference on Automated
  Planning and Scheduling (ICAPS~2014)}. AAAI, 2014 .

\bibitem{bryce-etal:2015:aaai}
Bryce D, Gao S, Musliner D, Goldman R.
\newblock SMT-Based Nonlinear {PDDL+} Planning.
\newblock In: \MCLabProceedingsOf{29th National Conference on Artificial
  Intelligence (AAAI~2015)}. AAAI, 2015 pp. 3247--3253.

\bibitem{bogomolov-etal:2014:aaai}
Bogomolov S, Magazzeni D, Podelski A, Wehrle M.
\newblock Planning as Model Checking in Hybrid Domains.
\newblock In: \MCLabProceedingsOf{28th National Conference on Artificial
  Intelligence (AAAI~2014)}. AAAI, 2014 pp. 2228--2234.

\bibitem{bogomolov-etal:2015:icaps}
Bogomolov S, Magazzeni D, Minopoli S, Wehrle M.
\newblock {PDDL+} Planning with Hybrid Automata: Foundations of Translating
  Must Behavior.
\newblock In: \MCLabProceedingsOf{25th International Conference on Automated
  Planning and Scheduling (ICAPS~2015)}. AAAI, 2015 pp. 42--46.

\bibitem{dellapenna-etal:2009:icaps}
Della~Penna G, Magazzeni D, Mercorio F, Intrigila B.
\newblock UPMurphi: A Tool for Universal Planning on {PDDL+} Problems.
\newblock In: \MCLabProceedingsOf{19th International Conference on Automated
  Planning and Scheduling (ICAPS~2009)}. AAAI, 2009 .

\bibitem{dellapenna-etal:2010:planning}
Della~Penna G, Intrigila B, Magazzeni D, Mercorio F.
\newblock Planning for Autonomous Planetary Vehicles.
\newblock In: \MCLabProceedingsOf{6th International Conference on Autonomic and
  Autonomous Systems (ICAS~2010)}. IEEE, 2010 pp. 131--136.

\bibitem{dellapenna-etal:2013:eurjcontrol}
Della~Penna G, Intrigila B, Magazzeni D, Melatti I, Tronci E.
\newblock Cgmurphi: Automatic synthesis of numerical controllers for nonlinear
  hybrid systems.
\newblock \emph{European Journal of Control}, 2013.
\newblock \textbf{19}(1):14--36.

\bibitem{alimguzhin-etal:2017:tac}
Alimguzhin V, Mari F, Melatti I, Salvo I, Tronci E.
\newblock Linearizing Discrete-Time Hybrid Systems.
\newblock \emph{{IEEE} Transactions on Automatic Control}, 2017.
\newblock \textbf{62}(10):5357--5364.
\newblock \doi{10.1109/TAC.2017.2694559}.

\bibitem{mari-etal:2014:tosem}
Mari F, Melatti I, Salvo I, Tronci E.
\newblock Model Based Synthesis of Control Software from System Level Formal
  Specifications.
\newblock \emph{{ACM} Transactions on Software Engineering and Methodology},
  2014.
\newblock \textbf{23}(1):1--42.

\bibitem{mazo-etal:2010:cav}
Mazo M, Davitian A, Tabuada P.
\newblock {PESSOA}: A tool for embedded controller synthesis.
\newblock In: \MCLabProceedingsOf{22nd International Conference on Computer
  Aided Verification (CAV~2010)}, volume 6174 of \emph{Lecture Notes in
  Computer Science}. Springer, 2010 pp. 566--569.
\newblock \doi{10.1007/978-3-642-14295-6_49}.

\bibitem{rungger-etal:2016:hscc}
Rungger M, Zamani M.
\newblock {SCOTS}: A Tool for the Synthesis of Symbolic Controllers.
\newblock In: \MCLabProceedingsOf{19th ACM International Conference on Hybrid
  Systems: Computation and Control (HSCC~2016)}. ACM, 2016 pp. 99--104.
\newblock \doi{10.1145/2883817.2883834}.

\bibitem{li-etal:2008:icaps}
Li H, Williams B.
\newblock Generative Planning for Hybrid Systems Based on Flow Tubes.
\newblock In: \MCLabProceedingsOf{18th International Conference on Automated
  Planning and Scheduling (ICAPS~2008)}. AAAI, 2008 pp. 206--213.

\bibitem{mancini-etal:2014:smartgridcomm}
Mancini T, Mari F, Melatti I, Salvo I, Tronci E, Gruber J, Hayes B, Prodanovic
  M, Elmegaard L.
\newblock Demand-Aware Price Policy Synthesis and Verification Services for
  Smart Grids.
\newblock In: \MCLabProceedingsOf{2014 IEEE International Conference on Smart
  Grid Communications (SmartGridComm~2014)}. IEEE, 2014 pp. 794--799.
\newblock \doi{10.1109/SmartGridComm.2014.7007745}.

\bibitem{mancini-etal:2015:dsd}
Mancini T, Mari F, Melatti I, Salvo I, Tronci E, Gruber J, Hayes B, Prodanovic
  M, Elmegaard L.
\newblock User Flexibility Aware Price Policy Synthesis for Smart Grids.
\newblock In: \MCLabProceedingsOf{18th Euromicro Conference on Digital System
  Design (DSD~2015)}. IEEE, 2015 pp. 478--485.
\newblock \doi{10.1109/DSD.2015.35}.

\bibitem{hayes-etal:2016:tsg}
Hayes B, Melatti I, Mancini T, Prodanovic M, Tronci E.
\newblock Residential Demand Management using Individualised Demand Aware Price
  Policies.
\newblock \emph{{IEEE} Transactions on Smart Grid}, 2017.
\newblock \textbf{8}(3).
\newblock \doi{10.1109/TSG.2016.2596790}.

\bibitem{lipovetzky-etal:2015:ijcai}
Lipovetzky N, Ramirez M, Geffner H.
\newblock Classical Planning with Simulators: Results on the Atari Video Games.
\newblock In: \MCLabProceedingsOf{24th International Join Conference on
  Artificial Intelligence (IJCAI~2015)}, volume~15. 2015 pp. 1610--1616.

\bibitem{ramirez-etal:2017:ijcai}
Ramirez M, Papasimeon M, Benke L, Lipovetzky N, Miller T, Pearce A.
\newblock Real--Time {UAV} Maneuvering via Automated Planning in Simulations.
\newblock In: \MCLabProceedingsOf{26th International Join Conference on
  Artificial Intelligence (IJCAI~2017)}. 2017 pp. 5243--5245.

\bibitem{frances-etal:2017:ijcai}
Frances G, Ram{\'\i}rez~J{\'a}vega M, Lipovetzky N, Geffner H.
\newblock Purely Declarative Action Descriptions are Overrated: Classical
  Planning with Simulators.
\newblock In: Proceedings of 26th International Joint Conference on Artificial
  Intelligence (IJCAI~2017). 2017 pp. 4294--4301.

\bibitem{lipovetzky-etal:2012:ecai}
Lipovetzky N, Geffner H.
\newblock Width and Serialization of Classical Planning Problems.
\newblock In: Proceedings of 20th European Conference on Artificial
  Intelligence (ECAI~2012). IOS Press, 2012 pp. 540--545.

\end{thebibliography}


==> content.tex <==
%!TEX root = ./root.tex
\AcronymResetAll

\clearpage
\tableofcontents
\clearpage

\AcronymResetAll

\section{Introduction}
\AcronymResetAll
\label{sec:introduction}
\Input[01.introduction]{content.tex}

\section{Formal framework}
\AcronymResetAll
\label{sec:preliminaries}
\Input[03.preliminaries]{content.tex}

\section{Case study: downregulation in assisted reproduction treatments}
\AcronymResetAll
\label{sec:treatment}
\Input[04.treatment]{content.tex}

\section{Computing optimal personalised treatments}
\AcronymResetAll
\label{sec:computing}
\Input[05.treatment-design]{content.tex}

\section{Multi-arm \Acl{ISCT}}
\AcronymResetAll
\label{sec:experiments}
\Input[07.experimental-results]{content.tex}

\section{Related work}
\AcronymResetAll
\label{sec:state-of-the-art}
\Input[02.state-of-the-art]{content.tex}

\section{Conclusions}
\AcronymResetAll
\label{sec:conclusions}
\Input[08.conclusions]{content.tex}

\subsubsection*{Acknowledgements}
We are grateful to the co-authors of the preliminary work in \cite{mancini-etal:2018:rcra-treatment}.

This work was partially supported by the following research projects/grants: 
%
Sapienza University 2018 project RG11816436BD4F21 ``Computing Complete Cohorts of Virtual Phenotypes for In Silico Clinical Trials and Model-Based Precision Medicine'';
Italian Ministry of University \& Research (MIUR) grant ``Dipartimenti di Eccellenza 2018--2022'' (Dept.\ Computer Science, Sapienza Univ.\ of Rome); 
EC FP7 project PAEON (Model Driven Computation of Treatments for Infertility Related Endocrinological Diseases, 600773);
INdAM ``GNCS Project 2019''; 
CINECA Class C ISCRA Project no.\ HP10CPJ9LW.

Clinical data used were gathered during a study conducted within EU FP7 Project PAEON. This study has been registered in \href{clin.trial.gov}{clin.trial.gov} (\href{https://clinicaltrials.gov/ct2/show/NCT02098668}{NCT02098668}).

%\bibliographystyle{fundam}
%\bibliography{...}
\Input{bibliography.tex} % root.bbl renamed into bibliography.tex


==> titlepage.tex <==
%!TEX root = root.tex

\title{%
	Optimal Personalised Treatment Computation through {\itshape In Silico} Clinical Trials on Patient Digital Twins%
	\thanks{This is a greatly extended and revised version
  		of the preliminary work presented in~\cite{mancini-etal:2018:rcra-treatment}. Authors equally contributed to this article.}
  	\thanks{This article should be cited as: Stefano Sinisi, Vadim Alimguzhin, Toni Mancini, Enrico Tronci, Federico Mari, Brigitte Leeners.
Optimal personalised treatment computation through in silico clinical trials on patient digital twins.
Fundamenta Informaticae, 174(3-4), pages 283-310, 2020.
DOI: 10.3233/FI-2020-1943}
}
\runninghead{S. Sinisi et al.}{%
	Optimal Personalised Treatment Computation through \Acsp{ISCT} on Patient Digital Twins%
}

\address{\url{sinisi@di.uniroma1.it}}

\author{%
Stefano Sinisi\corresponding, Vadim Alimguzhin, Toni Mancini,
Enrico Tronci\\
Computer Science Department\\
Sapienza University of Rome, Italy
\and
Federico Mari\\
Department of Movement, Human and Health Sciences\\
University of Rome Foro Italico, Italy
\and
Brigitte Leeners\\
Division of Reproductive Endocrinology\\
University Hospital Zurich, Switzerland
}


